QUALS: Corpus Equilibrium for Universal Forecasting via Pattern Quantization and Learnability Synchronization

Ubiquitous time series data across diverse domains enables critical applications in areas such as transportation systems and power grids. Recently, training foundation models on massive datasets to achieve accurate zero-shot forecasting has emerged as a major research focus. However, current studies predominantly prioritize architectural innovations while insufficiently addressing data diversity, often relying on simple data sampling strategies that fail to manage complex data distributions effectively, leading to inefficient use of training data and suboptimal performance. To address this, we propose QUALS, a large-scale time series corpus equilibrium framework. QUALS significantly enhances data efficiency, i.e., enabling existing models to achieve superior performance using only a small fraction of the original training data. Specifically, QUALS operates through two core mechanisms. First, a pattern quantization framework systematically decodes heterogeneous patterns from mixed corpora via vector quantization and uniform binning. Second, a learnability synchronization framework calibrates sampling weights for heterogeneous patterns, bridging the optimization gap between simple and complex motifs to maximize overall training efficiency. Extensive benchmarks demonstrate that pre-training on QUALS consistently achieves superior zero-shot performance, even under substantially reduced training budgets.

==> sections/exp_tsfm_results.tex <==
\rev{\mypara{TSFM-Bench.} Table~\ref{tab:benchmark_merged} further reports TSFM-Bench results using MAE and MSE Skill Scores. Official pre-training corpora and BLAST partially leak TSFM-Bench test data, while QUALS remains strictly leakage-free. Nevertheless, QUALS-trained variants achieve the highest Skill Scores across all metrics and model families. Most strikingly, they rescue leakage-advantaged TimeMoE models that fall below Seasonal Naive and improve Skill Scores over original Chronos and MOIRAI checkpoints by \textbf{11\% to 50\%}, while also systematically eclipsing their BLAST counterparts.}


==> sections/exp_tsfm_table.tex <==
\input{tables/tsfm_bench_main}


==> sections/experiments_old.tex <==

\section{Experiments}
We evaluate QUALS by retraining representative universal forecasters and assessing their zero-shot performance across large-scale benchmarks and systematic ablations.

\subsection{Experimental Setup}
\noindent\textbf{\textbf{Baselines}}
\label{subsection:baselines}
We evaluate six models: the base and large versions of TimeMoE~\cite{shi2024timemoe} and MOIRAI~\cite{woo2024moirai}, and the small and base versions of Chronos\footnote{We employ the Chronos-Bolt release.}. Models without superscripts use official open-source checkpoints. Superscript B denotes BLAST-based versions~\footnote{https://huggingface.co/datasets/ZezhiShao/BLAST}, trained on an 81.1B corpus curated from a 321B raw corpus with potentially untraceable leakage. Superscript Q denotes models trained from scratch on QUALS, using an 81.89B candidate corpus constructed from a strictly leakage-free 239B raw corpus collected from GIFT-Eval Pre-training datasets~\footnote{https://huggingface.co/datasets/Salesforce/GiftEvalPretrain} and synthetic data~\cite{ansari2024chronos}. Training protocols otherwise follow the original implementations, with only batch size and gradient accumulation adjusted for TimeMoE-large to fit 4$\times$L40 GPUs. Notably, Stage~3 synchronization in QUALS enables convergence with fewer updates than the original settings.

\noindent\textbf{Benchmarks \& Data Leakage Declaration.}
To ensure fair and rigorous evaluation, we categorize our benchmarks based on their data leakage status (i.e., whether test sets inadvertently appeared in official pre-training corpora)~\cite{shi2024timemoe, woo2024moirai, ansari2024chronos}:

\begin{itemize}[leftmargin=*, topsep=0pt, itemsep=2pt]
\item \textbf{Strictly Leakage-Free:} ARIES-TEST\footnote{https://huggingface.co/spaces/Blisky-li/ARIES-TEST}~\cite{wang2025aries}, BLAST-configured GIFT-Eval~\cite{gifteval}.
\item \textbf{Leakage-Present (Declared):} We explicitly identify the following leakages: 
{\color{red}
(1) \textit{Long-term time series forecasting}~\cite{li2025apt}\footnote{https://github.com/GestaltCogTeam/BasicTS}, including ETTh1, ETTh2, ETTm1, ETTm2, and Weather, where Weather is leaked in {TimeMoE}; 
(2) \textit{Full GIFT-Eval}\footnote{https://huggingface.co/spaces/Salesforce/GIFT-Eval}, which is partially leaked in {TimeMoE}$^B$, {TimeMoE}, {MOIRAI}$^B$, {Chronos}$^B$, and {Chronos}; 
(3) \textit{FEV-Bench}\footnote{https://huggingface.co/spaces/autogluon/fev-bench}~\cite{shchur2025fev}, which is partially leaked in {TimeMoE}$^B$, {TimeMoE}, {MOIRAI}$^B$, {MOIRAI}, and {Chronos}$^B$.
% 
These benchmarks are not leaked in QUALS-based retrained models.}
\end{itemize}


\noindent\textbf{Metrics}
We report Mean Squared Error~(MSE) and Mean Absolute Error~(MAE) as the primary metrics in the main experiments. Under the regular setting, we report the mean and median values of MAE and MSE on ARIES-TEST. For GIFT-EVAL, we adopt Mean Absolute Scaled Error~(MASE) and Continuous Ranked Probability Score~(CRPS). For FEV-Bench, we report Scaled Quantile Loss~(SQL), Mean Absolute Scaled Error~(MASE), Weighted Quantile Loss~(WQL), and Weighted Absolute Percentage Error~(WAPE), all measured as skill scores relative to Seasonal Naive~\cite{makridakis2020m4}.


\subsection{Benchmark Comparison Experiment}
\noindent\textbf{Long-term Time Series Forecasting.} As presented in Table~\ref{tab:main_result}, models pre-trained on the QUALS corpus demonstrate consistent improvements of 3\% to 20\% (MSE/MAE) over their official open-source checkpoints. Compared to BLAST-balanced counterparts, QUALS achieves an additional 5–10\% MSE reduction in specific scenarios (e.g., Chronos on ETTh1, TimeMoE on ETTh2 and ETTm1/2). Crucially, QUALS maintains a decisive lead even on the notoriously stable Weather dataset. Overall, QUALS secures the lowest errors across the most horizons, proving that corpus equilibrium translates directly into stronger long-term zero-shot forecasts.

\noindent\textbf{ARIES TEST.} Table~\ref{tab:ARIES} presents the results on ARIES TEST, a synthetic benchmark encompassing diverse intrinsic temporal properties. While baselines struggle with these varied patterns, QUALS demonstrates remarkable superiority, surpassing the original MOIRAI by over 60\% in MSE.  This substantial improvement provides compelling evidence that the strategic equilibrium between pattern distribution and learnability effectively enables robust zero-shot forecasting capabilities.

\noindent\textbf{BLAST-configured GIFT-Eval.} To ensure a fair comparison free from the severe data leakage prevalent in massive pre-training corpora, we evaluate on the leakage-free BLAST-configured GIFT-Eval (Table~\ref{tab:gift_eval}). Under this rigorous setting, QUALS models deliver relative error reductions of \textbf{7\% to 22\%} (MASE/CRPS) compared to their original versions, and yield an additional \textbf{1\% to 9\%} performance gain over the BLAST framework across all architectures.

\noindent\textbf{Full GIFT-Eval.} We further evaluate on the full 97-task GIFT-Eval (Table~\ref{tab:gift_eval_all}).
In this setting, official corpora and BLAST models inherently possess an unfair memorization advantage due to explicit downstream data leakage. Astonishingly, despite using a strictly leakage-free and substantially smaller training budget, QUALS consistently outperforms all baselines. Most strikingly, it reduces the MASE of the leakage-advantaged TimeMoE models by \textbf{17\% to 23\%}, alongside consistent wins for Chronos and MOIRAI.

\noindent\textbf{FEV-Bench.} Table~\ref{tab:fev} reports FEV-Bench results using Skill Scores (relative improvement over Seasonal Naive). Notably, the official pre-training corpora and BLAST explicitly leak FEV-Bench test data. Specifically, the official MOIRAI corpus exhibits a severe \textbf{28\%} test leakage, causing BLAST variants to underperform the originals as balanced sampling inadvertently dilutes this unfair advantage. Nevertheless, QUALS-trained variants overcome this disadvantage to systematically eclipse both the original and BLAST counterparts. 
% 
They achieve the highest Skill Scores across all metrics, outperforming the leakage-advantaged original models by 9\% to 18\% and systematically eclipsing their BLAST counterparts.
% They achieve the highest Skill Scores across all metrics, outperforming the leakage-advantaged original models by up to \textbf{9\% to 18\%} and systematically eclipse their BLAST counterparts.


% Preamble:
% \usepackage{booktabs}

% Preamble:
% \usepackage{booktabs}
% \usepackage{multirow}

% Preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{xcolor} % and define MyRed2 if not defined

\begin{table*}[]
\setlength{\abovecaptionskip}{.2 cm}
\caption{
Performance comparison on the BLAST-configured GIFT-Eval benchmark.
Due to the experimental setup, we retain only the test data that do not exhibit data leakage.
Models with superior performance are highlighted in {\color{MyRed2}\textbf{red}}.
}
\setlength\tabcolsep{1.2pt}
\resizebox{1\linewidth}{!}{
\begin{tabular}{rr|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule[1.5pt]
\multicolumn{2}{l}{\textbf{Models}} & \multicolumn{1}{|l}{\textbf{TimeMoE}$_{l}^{\textbf{Q}}$} & \multicolumn{1}{l}{\textbf{TimeMoE}$_{l}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{TimeMoE}$_{l}$} &
 \multicolumn{1}{l}{\textbf{TimeMoE}$_{b}^{\textbf{Q}}$}
& \multicolumn{1}{l}{\textbf{TimeMoE}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{TimeMoE}$_{b}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{l}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{l}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{MOIRAI}$_{l}$} & 
\multicolumn{1}{l}{\textbf{MOIRAI}$_{b}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{MOIRAI}$_{b}$} 
&\multicolumn{1}{l}{\textbf{Chronos}$_{b}^{\textbf{Q}}$}
& \multicolumn{1}{l}{\textbf{Chronos}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{Chronos}$_{b}$} & 
\multicolumn{1}{l}{\textbf{Chronos}$_{s}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{Chronos}$_{s}^{\textbf{B}}$} & \multicolumn{1}{l}{\textbf{Chronos}$_{s}$} \\
\midrule
\multicolumn{2}{c|}{\textbf{MASE}$\downarrow$} & {\color{MyRed2}\textbf{0.677}}&\scalebox{1.1}0.742 & 0.872 & \scalebox{1.1}
{\color{MyRed2}\textbf{0.734}}&
0.760 & 0.888 & \scalebox{1.1}
{\color{MyRed2}\textbf{0.729}}&
0.740 & 0.816 & \scalebox{1.1}
{\color{MyRed2}\textbf{0.745}}&
0.759 & 0.812 & \scalebox{1.1}
{\color{MyRed2}\textbf{0.659}} &
0.682 & 0.724 & \scalebox{1.1}
{\color{MyRed2}\textbf{0.663}}&
0.684& 0.736 \\
\midrule
\multicolumn{2}{c|}{\textbf{CRPS}$\downarrow$} &
{\color{MyRed2}\textbf{0.557}} & 0.593 & 0.702&
{\color{MyRed2}\textbf{0.593}} & 0.616 & 0.706&
{\color{MyRed2}\textbf{0.576}} & 0.580 & 0.642&
{\color{MyRed2}\textbf{0.585}} & 0.614 & 0.641&
{\color{MyRed2}\textbf{0.450}} & 0.468  & 0.489&
{\color{MyRed2}\textbf{0.453}} & 0.470 & 0.485\\

\bottomrule[1.5pt]
\end{tabular}}
\label{tab:gift_eval}
\vspace{-5pt}
\end{table*}

\begin{table*}[]
\setlength{\abovecaptionskip}{.2 cm}
\caption{
Performance on full Gift-Eval benchmark
Models with superior performance are highlighted in {\color{MyRed2}\textbf{red}}.
}
\setlength\tabcolsep{1.2pt}
\resizebox{1\linewidth}{!}{
\begin{tabular}{rr|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule[1.5pt]
\multicolumn{2}{l}{\textbf{Models}} & \multicolumn{1}{|l}{\textbf{TimeMoE}$_{l}^{\textbf{Q}}$} & \multicolumn{1}{l}{\textbf{TimeMoE}$_{l}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{TimeMoE}$_{l}$} &
 \multicolumn{1}{l}{\textbf{TimeMoE}$_{b}^{\textbf{Q}}$}
& \multicolumn{1}{l}{\textbf{TimeMoE}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{TimeMoE}$_{b}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{l}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{l}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{MOIRAI}$_{l}$} & 
\multicolumn{1}{l}{\textbf{MOIRAI}$_{b}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{MOIRAI}$_{b}$} 
&\multicolumn{1}{l}{\textbf{Chronos}$_{b}^{\textbf{Q}}$}
& \multicolumn{1}{l}{\textbf{Chronos}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{Chronos}$_{b}$} & 
\multicolumn{1}{l}{\textbf{Chronos}$_{s}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{Chronos}$_{s}^{\textbf{B}}$} & \multicolumn{1}{l}{\textbf{Chronos}$_{s}$} \\
\midrule
\multicolumn{2}{c|}{\textbf{MASE}$\downarrow$} &{\color{MyRed2}\textbf{0.846}} & 0.852& 1.110& {\color{MyRed2}\textbf{0.881}}& 0.896& 1.067& {\color{MyRed2}\textbf{0.858}}& 0.880&  0.875&{\color{MyRed2}\textbf{0.888}}& 0.908& 	
0.901& {\color{MyRed2}\textbf{0.798}}& 0.804& 0.808& {\color{MyRed2}\textbf{0.803}}&0.809&0.822  \\
\midrule
\multicolumn{2}{c|}{\textbf{CRPS}$\downarrow$} & {\color{MyRed2}\textbf{0.723}}& 0.728& 0.882& {\color{MyRed2}\textbf{0.759}}& 0.766& 0.906& {\color{MyRed2}\textbf{0.580}}& 0.598& 0.599& {\color{MyRed2}\textbf{0.608}}& 0.623& 0.610& {\color{MyRed2}\textbf{0.568}}& 0.574& 0.574 & {\color{MyRed2}\textbf{0.571}}& 0.574& 0.577 \\

\bottomrule[1.5pt]
\end{tabular}}
\label{tab:gift_eval_all}
\end{table*}



\begin{table*}[]
\setlength{\abovecaptionskip}{.2 cm}
\vspace{-5pt}
\caption{
Performance of Skill Score on Fev benchmark
Models with superior performance are highlighted in {\color{MyRed2}\textbf{red}}.
}
\setlength\tabcolsep{1.2pt}
\resizebox{1\linewidth}{!}{
\begin{tabular}{rr|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule[1.5pt]
\multicolumn{2}{l}{\textbf{Models}} & \multicolumn{1}{|l}{\textbf{TimeMoE}$_{l}^{\textbf{Q}}$} & \multicolumn{1}{l}{\textbf{TimeMoE}$_{l}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{TimeMoE}$_{l}$} &
 \multicolumn{1}{l}{\textbf{TimeMoE}$_{b}^{\textbf{Q}}$}
& \multicolumn{1}{l}{\textbf{TimeMoE}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{TimeMoE}$_{b}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{l}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{l}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{MOIRAI}$_{l}$} & 
\multicolumn{1}{l}{\textbf{MOIRAI}$_{b}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{MOIRAI}$_{b}$} 
&\multicolumn{1}{l}{\textbf{Chronos}$_{b}^{\textbf{Q}}$}
& \multicolumn{1}{l}{\textbf{Chronos}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{Chronos}$_{b}$} & 
\multicolumn{1}{l}{\textbf{Chronos}$_{s}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{Chronos}$_{s}^{\textbf{B}}$} & \multicolumn{1}{l}{\textbf{Chronos}$_{s}$} \\
\midrule
\multicolumn{2}{c|}{\textbf{SQL}$\uparrow$}  &{\color{MyRed2}\textbf{0.102}}&0.086&0.035 &{\color{MyRed2}\textbf{0.094}}&0.059& 0.032&{\color{MyRed2}\textbf{0.360}}&0.303&0.351&{\color{MyRed2}\textbf{0.350}}&0.292&0.321 &{\color{MyRed2}\textbf{0.393}}&0.386& 0.389&{\color{MyRed2}\textbf{0.391}}&0.382&0.378 \\
\midrule
\multicolumn{2}{c|}{\textbf{MASE}$\uparrow$}  &{\color{MyRed2}\textbf{0.110}}&0.095& 0.044&{\color{MyRed2}\textbf{0.102}}&0.067&0.040 &{\color{MyRed2}\textbf{0.226}}&0.151& 0.216&{\color{MyRed2}\textbf{0.214}}&0.140& 0.181&{\color{MyRed2}\textbf{0.275}}&0.266& 0.265&{\color{MyRed2}\textbf{0.275}}&0.260&0.256\\
\midrule
\multicolumn{2}{c|}{\textbf{WQL}$\uparrow$}  &{\color{MyRed2}\textbf{0.138}}&0.113&0.088 &{\color{MyRed2}\textbf{0.123}}&0.097&0.070 &0.398&0.352& {\color{MyRed2}\textbf{0.405}}&{\color{MyRed2}\textbf{0.388}}&0.338& 0.374&{\color{MyRed2}\textbf{0.437}}&0.428& 0.432&{\color{MyRed2}\textbf{0.430}}&0.422&0.422 \\
\midrule
\multicolumn{2}{c|}{\textbf{WAPE}$\uparrow$} 
 &{\color{MyRed2}\textbf{0.125}}&0.100&0.075 &{\color{MyRed2}\textbf{0.109}}&0.083&0.056 &0.247&0.192& {\color{MyRed2}\textbf{0.259}}&{\color{MyRed2}\textbf{0.236}}&0.175& 0.228&{\color{MyRed2}\textbf{0.307}}&0.296& 0.298&{\color{MyRed2}\textbf{0.303}}&0.287&0.290\\

\bottomrule[1.5pt]
\end{tabular}}
\label{tab:fev}
\end{table*}
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{0.9}
\caption{Rogressive ablation of QUALS by cumulatively removing components from Stage 3 to Stage 1.}
\label{tab:ablation_transposed_quals_321_best}

\resizebox{\textwidth}{!}{%
\begin{tabular}{l l ccccc ccccc ccccc ccccc}
\toprule[1.5pt]
\multicolumn{2}{c}{} &
\multicolumn{5}{c}{\textbf{QUALS}} &
\multicolumn{5}{c}{\textbf{w/o Stage3} (Candidate Corpus)} &
\multicolumn{5}{c}{\textbf{w/o Stage2} (Codebook Sample)} &
\multicolumn{5}{c}{\textbf{w/o Stage1} (BLAST)} \\
\cmidrule(lr){3-7}\cmidrule(lr){8-12}\cmidrule(lr){13-17}\cmidrule(lr){18-22}
\textbf{MODEL} & \textbf{Metric} &
ETTh1 & ETTh2 & ETTm1 & ETTm2 & Weather &
ETTh1 & ETTh2 & ETTm1 & ETTm2 & Weather &
ETTh1 & ETTh2 & ETTm1 & ETTm2 & Weather &
ETTh1 & ETTh2 & ETTm1 & ETTm2 & Weather \\
\midrule

\multirow{2}{*}{\textbf{ChronosBolt}$_s$} & MSE$\downarrow$ &
{\color{MyRed2}\textbf{0.382}} & {\color{MyRed2}\textbf{0.346}} & {\color{MyRed2}\textbf{0.371}} & 0.287 & {\color{MyRed2}\textbf{0.243}} &
0.397 & 0.354 & 0.386 & 0.285 & {\color{MyRed2}\textbf{0.243}} &
0.419 & 0.362 & 0.405 & {\color{MyRed2}\textbf{0.278}} & 0.247 &
0.411 & 0.358 & 0.404 & 0.282 & 0.249 \\
& MAE$\downarrow$ &
{\color{MyRed2}\textbf{0.399}} & {\color{MyRed2}\textbf{0.373}} & 0.381 & 0.321 & 0.263 &
0.402 & 0.381 & {\color{MyRed2}\textbf{0.379}} & 0.314 & {\color{MyRed2}\textbf{0.262}} &
0.412 & 0.384 & 0.384 & {\color{MyRed2}\textbf{0.313}} & 0.264 &
0.409 & 0.382 & 0.382 & 0.316 & 0.268 \\
\midrule

\multirow{2}{*}{\textbf{ChronosBolt}$_b$} & MSE$\downarrow$ &
{\color{MyRed2}\textbf{0.391}} & {\color{MyRed2}\textbf{0.349}} & {\color{MyRed2}\textbf{0.390}} & {\color{MyRed2}\textbf{0.275}} & {\color{MyRed2}\textbf{0.240}} &
0.393 & 0.352 & 0.401 & 0.280 & 0.248 &
0.404 & 0.350 & 0.397 & 0.282 & 0.259 &
0.409 & 0.355 & 0.390 & 0.277 & 0.244 \\
& MAE$\downarrow$ &
{\color{MyRed2}\textbf{0.401}} & {\color{MyRed2}\textbf{0.374}} & 0.379 & {\color{MyRed2}\textbf{0.313}} & {\color{MyRed2}\textbf{0.259}} &
0.403 & 0.380 & 0.381 & 0.321 & 0.269 &
0.410 & 0.381 & 0.384 & 0.322 & 0.281 &
0.409 & 0.377 & {\color{MyRed2}\textbf{0.375}} & {\color{MyRed2}\textbf{0.313}} & 0.263 \\
\midrule

\multirow{2}{*}{\textbf{TimeMoE}$_b$} & MSE$\downarrow$ &
{\color{MyRed2}\textbf{0.383}} & {\color{MyRed2}\textbf{0.338}} & {\color{MyRed2}\textbf{0.354}} & {\color{MyRed2}\textbf{0.251}} & 0.248 &
0.398 & 0.341 & 0.360 & 0.254 & {\color{MyRed2}\textbf{0.242}} &
0.405 & {\color{MyRed2}\textbf{0.338}} & 0.363 & 0.269 & 0.255 &
0.399 & 0.356 & 0.394 & 0.274 & 0.244 \\
& MAE$\downarrow$ &
{\color{MyRed2}\textbf{0.405}} & 0.384 & {\color{MyRed2}\textbf{0.378}} & {\color{MyRed2}\textbf{0.316}} & 0.282 &
0.407 & {\color{MyRed2}\textbf{0.382}} & 0.382 & 0.318 & {\color{MyRed2}\textbf{0.274}} &
0.416 & 0.383 & 0.381 & 0.319 & 0.288 &
0.412 & 0.391 & 0.399 & 0.326 & 0.278 \\
\bottomrule[1.5pt]
\end{tabular}%
}
\end{table*}


\begin{figure}[h]
  \centering
  \includegraphics[width=0.85\linewidth]{figures/quals_xr.pdf}
  \vspace{-10pt}
  \caption{Impact of Stage 2 Bin Granularity of ECDF}
  \label{fig:xr}
  \vspace{-10pt}
\end{figure}


\subsection{Ablation Study}
Table~\ref{tab:ablation_transposed_quals_321_best} presents a stepwise ablation study validate the role of each QUALS component. Removing Stage 3 (Learnability Synchronization) consistently increases forecasting errors, proving that mere distribution balancing is insufficient.
% 
Further removing Stage 2 (Pattern Binning) and relying instead on naive codebook sampling exacerbates the degradation, confirming that our spectral discretization is vital to prevent long-tail motif loss. Finally, replacing Stage 1's VQ-SwinTTS with BLAST's statistical heuristics yields the worst performance. This demonstrates that deep semantic quantization captures temporal morphologies far more effectively than rigid mathematical metrics.

Figure~\ref{fig:xr} illustrates the sensitivity to the number of pattern bins ($M$) in Stage 2, evaluated under a fixed total training volume. We observe a distinct U-shaped trade-off: a small $M$ (e.g., 200) causes under-fitting by collapsing diverse motifs into coarse bins, whereas excessive bins ($>5000$) lead to over-fragmentation and data sparsity. Optimal performance occurs between 2,000 and 4,000 bins, where QUALS successfully hits the "sweet spot" balancing high-resolution pattern coverage and sufficient sampling density.

{\color{red}Move figure 9 to here}

\begin{table}[h]
\centering
\caption{QUALS vs. BLAST: Scale and Efficiency.}
\vspace{-10pt}
\small
\label{tab:quals_blast_efficiency}
\begin{tabular}{c|c|c}
\toprule
\textbf{Metric} & \textbf{QUALS} & \textbf{BLAST} \\
\midrule
Raw Corpus Scale      &239 B  & 321 B \\
Curated Corpus Scale      &81.89 B  & 81.10 B  \\
\midrule
Representation Time          & 20 GPU-hours &  336 CPU-hours\\
Sampling Time                 & 12 CPU-hours  & 18 CPU-hours \\
Rebalancing Time         & 7 GPU-hours &  -\\
\bottomrule
\end{tabular}
\vspace{-5pt}
\end{table}

% Requires: \usepackage{booktabs}
% Optional (nice alignment): \usepackage{siunitx}

% Requires: \usepackage{booktabs}


\begin{table}[t]
\centering
\caption{Zero-Shot performance (MSE / MAE) across 5 benchmarks in Table~2 and their training efficiency (tokens). 
Bottom value represents the pre-training token budget (Billions, B). 
"-" indicates token count not reported.}
\label{tab:performance_efficiency}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{l|c|c|c}
\toprule
\textbf{Model} & \textbf{QUALS (Ours)} & \textbf{BLAST} & \textbf{Official Baseline} \\
\midrule

% Chronos-Small
\textbf{ChronosBolt-Small} & 
\color{MyRed2}\textbf{\splitcell{0.326 / 0.347}{61.86 B}} & 
\splitcell{0.341 / 0.352}{104.85 B} & 
\splitcell{0.358 / 0.360}{-} 
\\ \midrule

% Chronos-Base
\textbf{ChronosBolt-Base} & 
\color{MyRed2}\textbf{\splitcell{0.329 / 0.345}{125.82 B}} & 
\splitcell{0.335 / 0.347}{167.77 B} & 
\splitcell{0.351 / 0.351}{-} 
\\ \midrule

% MOIRAI-Base
\textbf{MOIRAI-Base} & 
\color{MyRed2}\textbf{\splitcell{0.332 / 0.349}{4.42 B}} & 
\splitcell{0.338 / 0.353}{6.55 B} & 
\splitcell{0.357 / 0.361}{6.55 B} 
\\ \midrule

% MOIRAI-Large
\textbf{MOIRAI-Large} & 
\color{MyRed2}\textbf{\splitcell{0.327 / 0.344}{4.83 B}} & 
\splitcell{0.335 / 0.350}{6.55 B} & 
\splitcell{0.381 / 0.393}{6.55 B} 
\\ \midrule

% TimeMoE-Base
\textbf{TimeMoE-Base} & 
\color{MyRed2}\textbf{\splitcell{0.315 / 0.353}{26.20 B}} & 
\splitcell{0.333 / 0.361}{78.64 B} & 
\splitcell{0.350 / 0.381}{419.43 B} 
\\ \midrule

% TimeMoE-Large
\textbf{TimeMoE-Large} & 
\color{MyRed2}\textbf{\splitcell{0.314 / 0.352}{99.61 B}} & 
\splitcell{0.330 / 0.360}{209.71 B} & 
\splitcell{0.352 / 0.380}{419.43 B} 
\\ \bottomrule

\end{tabular}%
}
\end{table}

\subsection{Efficiency Analysis}\label{Efficiency}
\noindent\textbf{Data Scale \& Constraints.} Early paradigms assume that scaling inherently improves performance, leading BLAST to aggregate a $\sim$321B corpus (Table~\ref{tab:quals_blast_efficiency}). To strictly prevent data leakage, QUALS restricts its raw corpus to $\sim$239B points. Moreover, all expanded corpora can be processed via VQ-SwinTTS inference instead of requiring costly statistical computations.

\noindent\textbf{Stage-wise Processing Efficiency.} Building upon the computational accounting detailed in Section~\ref{pipeline}, we compare the end-to-end efficiency of QUALS and BLAST, as summarized in Table~\ref{tab:quals_blast_efficiency}. The fundamental advantage of QUALS lies in its paradigm shift from CPU-bound mathematical heuristics to a highly scalable, GPU-accelerated pipeline.

Specifically, BLAST's reliance on statistical feature extraction incurs a prohibitive 336 CPU-hours on server-grade hardware and scales poorly to massive datasets. Furthermore, its high-complexity UMAP dimensionality reduction forces it to aggressively down-sample and train on merely 1\% of the raw corpus, causing irreversible information loss. In contrast, QUALS bypasses these bottlenecks entirely. By replacing CPU-intensive feature engineering with rapid VQ-SwinTTS inference and substituting UMAP with efficient PCA and ECDF, QUALS processes the full 239B corpus in a strictly lossless manner. Even with the introduction of the novel learnability synchronization stage (Stage~3), the marginal overhead remains remarkably low ($\sim$7 GPU-hours). Ultimately, QUALS reduces the end-to-end preparation timeframe from weeks to under two days while eliminating the compromises introduced by down-sampling, thereby establishing a robust foundation for billion-scale pre-training.

\noindent\textbf{Pre-training Budget Efficiency}
Table~\ref{tab:performance_efficiency} challenges the conventional scaling law for universal time series forecasting by demonstrating that \textbf{QUALS} achieves superior zero-shot accuracy with drastically reduced data volume. Most notably, for \textbf{TimeMoE-Base}, QUALS achieves a significantly lower MSE~(0.315 vs.\ 0.350) using only \textbf{26.20B} tokens---a \textbf{16$\times$ reduction} compared to the official 419.43B budget. This implies that over 90\% of the training tokens constitute redundant patterns that yield diminishing returns. This efficiency gain is consistent across architectures: \textbf{ChronosBolt-Small} reduces the token budget by \textbf{40\%} compared to BLAST while improving MSE by 4.4\%, and \textbf{MOIRAI-Large} outperforms its official checkpoint and the BLAST counterpart with 26\% fewer tokens. These results confirm that optimizing corpus equilibrium in terms of pattern distribution and learnability, rather than merely increasing scale, establishes a far more efficient paradigm for pre-training.


==> sections/introduction_old.tex <==

\section{Introduction}
% Universal time series forecasting has gained prominence for its robust zero-shot capabilities. While current research primarily pursues architectural innovation and indiscriminately scales pretraining data~\cite{ansari2024chronos, ansari2025chronos2, liu2024timer}, evidence from NLP~\cite{DBLP:journals/corr/abs-2001-08361, xie2023data} and CV~\cite{deng2009imagenet, zeng2024understanding} explicitly demonstrate that data diversity~\cite{chan2022data, lee2022deduplicating} and quality~\cite{hoffmann2022training, lei2023comprehensive} are far more critical than mere scale for robust generalization.

Time series data are ubiquitous across diverse real-world domains~\cite{shi2024timemoe, gao2024building, goswami2024moment}. Recently, universal time series forecasting has gained tremendous prominence for its robust zero-shot generalization capabilities. Its fundamental paradigm relies on training large-scale models on massive datasets to induce the emergence of zero-shot abilities. Although current research has achieved remarkable success through continuous architectural innovations~\cite{ansari2024chronos, ansari2025chronos2, liu2024timer}, consensus from Natural Language Processing~(NLP)~\cite{DBLP:journals/corr/abs-2001-08361, xie2023data} and Computer Vision~(CV)~\cite{deng2009imagenet, zeng2024understanding} explicitly demonstrates that data diversity~\cite{chan2022data, lee2022deduplicating} and validity~\cite{hoffmann2022training, lei2023comprehensive} are far more critical than mere data scale.

%As time-series corpora from diverse domains such as nature, health, and web~\cite{shi2024timemoe, gao2024building, goswami2024moment} scale to hundreds of billions, efficient data utilization emerges as the primary system-level bottlenecks restricting universal forecasting. Naive or stratified sampling~\cite{woo2024moirai, liu2024moiraimoe} based on datasets and domains from raw corpora inevitably triggers severe long-tail biases, causing models to \textit{overfit pervasive patterns but underfit rare yet critical ones}. As contrasted in Figure~\ref{fig:intro}, while statistical heuristics~\cite{wang2025aries} like BLAST~\cite{shao2025blast, shao2024exploring} attempt to equalize pattern quantities by sampling predefined properties such as trends and stationarity, they suffer from critical bottlenecks:

% \begin{itemize}[leftmargin=*, nosep]
    %\item \textbf{Incomplete Coverage \& Prohibitive Overhead:} Rigid statistics fail to index detailed temporal features~\cite{wang2025aries}. Furthermore, extracting these features across massive corpora consumes weeks of CPU time, rendering such heuristics fundamentally unscalable.
    %\item \textbf{Ignored Learnability Discrepancy:} Static quantity balancing completely ignores optimization dynamics~\cite{fu2025selective, yang2025not}. Simple patterns inevitably dominate gradients, causing models to overfit fast converging signals and underfit complex ones.
    %\item \textbf{Unregulated Data Leakage:} Indiscriminate aggregation of public data overlaps with benchmarks~\cite{gifteval, fev}, introducing opaque leakage that erodes evaluation integrity and actual reliability.
%\end{itemize}

As illustrated in Figure~\ref{fig:intro}~(a), the current corpus curation pipeline for universal forecasting typically operates as follows: researchers tend to aggregate open-source time series data across diverse domains, blindly adhering to the scaling laws from Large Language Models~(LLMs)~\cite{gruver2023large, sun2025xihe} to indiscriminately expand data volume. For instance, while Chronos~\cite{ansari2024chronos} initially utilized a mere 84B training tokens, the recent TimeBench corpus has surged to a staggering 1000B~\cite{liu2025sundial}. Accompanied by bloated training budgets, such blind cross-domain aggregation not only incurs prohibitive computational waste but also exposes severe inefficiencies in data utilization.

The primary driver of this inefficiency lies in the severe imbalances of data distributions as shown in Figure~\ref{fig:intro}~(b). Crucially, whether relying on naive or domain-based stratified sampling~\cite{woo2024moirai, liu2024moiraimoe}, blindly expanding the macroscopic \textit{domains} of data sources does not inherently guarantee the diversity of microscopic temporal \textit{patterns}. For instance, meteorological data alone accounts for a staggering 87\% of the TimeMoE dataset~\cite{shi2024timemoe}, inevitably inducing an extreme long-tail distribution dominated by a single seasonality. This fundamental skew causes models to \textit{severely overfit pervasive patterns while critically underfitting rare yet vital ones}.

Although subsequent works such as BLAST~\cite{shao2025blast} attempt to alleviate distribution imbalances via heuristic pattern definitions, they still suffer from critical flaws in both representation and efficiency. On the one hand, rigid statistical metrics fail to accurately index deep and detailed temporal features~\cite{wang2025aries}, resulting in severely incomplete semantic coverage. On the other hand, extracting these heuristic features across massive corpora incurs prohibitive computational overhead, which often consumes weeks of CPU time and thereby renders such approaches fundamentally unscalable.

Furthermore, underlying temporal patterns are fundamentally inequivalent in nature, a critical reality completely overlooked by current paradigms. Simple, pure motifs are effortlessly captured and assimilated by models, whereas complex data interwoven with multiple frequencies or noise remain notoriously difficult to optimize~\cite{wang2025aries}. As illustrated in Figure~\ref{fig:intro}~(c), this intrinsic "learnability discrepancy" causes simple patterns to rapidly monopolize gradient descent updates during training, leaving challenging patterns persistently under-optimized and insufficiently fitted.

%These limitations highlight the demand for a principled, scalable, and leakage-free \textit{corpus construction and sampling layer}. To fundamentally resolve these curation bottlenecks shown in Figure~\ref{fig:intro}, we propose \textbf{QUALS} (Pattern \textbf{QUA}ntization \& \textbf{L}earn-ability \textbf{S}ynchronization), a \textbf{dual-equilibrium} time-series pre-train corpus construction framework that quantizes diverse patterns and synchronizes learnability to improve zero-shot forecasting. \textbf{For pattern diversity}, we leverage self-supervised learning to capture deep temporal semantics, specifically targeting local temporal features driven by the inherent continuity of data streams. \textbf{For pattern learnability}, rather than instance-level noise, we formulate it as the intrinsic optimization difficulty of pattern subsets, explicitly synchronizing their convergence rates during training


%QUALS comprises three progressive stages:(i) \textbf{Patch-level Pattern Discretization.} We propose the multi-scale \textbf{Vector-Quantized Swin Transformer for Time Series (VQ-SwinTTS)}~\cite{DBLP:conf/iccv/LiuL00W0LG21} to discretize local temporal semantics into a learnable, shared codebook~\cite{DBLP:conf/nips/OordVK17, DBLP:conf/aistats/LeeMA23}, obtaining data-driven patch embedding~\cite{nietime}.(ii) \textbf{Series-level Pattern Binning}. Discrete patches are lifted to a global pattern space via Codebook PCA~\cite{hotelling1933analysis} and spectrum-aware discretization~\cite{DBLP:journals/pami/JegouDS11}, ensuring uniform coverage across the latent patterns bins.(iii) \textbf{Learnability Synchronization}. On the candidate corpus, we employ Group Relative Policy Optimization~(GRPO) to estimate bin-wise convergence rates, dynamically aligning learning speeds to bridge the overfitting-underfitting gap.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.95\linewidth]{figures/intro2.pdf}
  \vspace{-5pt}
  \caption{Overview of existing corpus curation paradigms and their inherent flaws in pattern distribution and learnability imbalances.}
  \vspace{-5pt}
  \label{fig:intro}
\end{figure}

\begin{table}[htbp]
  \centering
  \caption{Comparison of different corpus curation paradigms.}
  \vspace{-5pt}
  \label{tab:comparison}
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{lccc}
    \toprule
    & \multirow{2}{*}{\textbf{QUALS (Ours)}} & \textbf{BLAST} & \textbf{Others} \\
    &  & \cite{shao2025blast} & \cite{ansari2024chronos,woo2024moirai,shi2024timemoe,liu2024timer} \\
    \midrule
    \textbf{Pattern Distribution} & Deep Data-Driven & Heuristic & Naive/Stratified \\
    \textbf{Pattern Learnability} & GRPO-Synchronized & $\times$ & $\times$ \\
    \bottomrule
  \end{tabular}%
  }
\end{table}


To fundamentally resolve these critical bottlenecks, we propose QUALS (Pattern \textbf{QUA}ntization \& \textbf{L}earnability \textbf{S}ynchronization). As contrasted in Table~\ref{tab:comparison}, unlike prior paradigms that rely on brute-force data accumulation or rigid heuristics, QUALS establishes a dual-equilibrium pre-training corpus curation framework that explicitly balances both pattern distribution and intrinsic learnability.

First, to overcome the representational bottlenecks and unscalable overhead of heuristic metrics, QUALS introduces a fully data-driven Pattern Discretization and Binning pipeline. Rather than relying on rigid statistical definitions or blindly expanding data domains, we employ a multi-scale quantization architecture~\cite{DBLP:conf/iccv/LiuL00W0LG21, DBLP:conf/nips/OordVK17, DBLP:conf/aistats/LeeMA23} coupled with spectrum-aware discretization~\cite{hotelling1933analysis, DBLP:journals/pami/JegouDS11} to map highly heterogeneous time series into a global, discrete pattern space. This data-driven transformation directly tackles the severe long-tail distribution inherent in raw corpora, grouping temporal semantics into uniformly distributed Pattern Bins in a high-fidelity manner. Consequently, it achieves a strict quantity equilibrium across diverse motifs, ensuring that rare but vital patterns are no longer overshadowed by pervasive ones.

Second, resolving the distribution imbalance alone does not counteract the intrinsic learnability discrepancy , where simple patterns inevitably dominate gradient updates. To correct this optimization bias, we pioneer a Learnability Synchronization mechanism. By leveraging offline Group Relative Policy Optimization~(GRPO)~\cite{fu2025reward} to profile bin-wise convergence rates throughout a proxy training lifecycle , this stage adaptively recalibrates sampling weights to penalize fast-learning motifs and prioritize challenging ones. This synchronization aligns the learning progress across the corpus , effectively alleviating the gap between overfitting simple sequences and underfitting complex ones. Ultimately, this aware rebalancing avoids redundant updates and significantly compresses pre-training costs.
%Moreover, to strictly prevent data leakage prevalent in existing universal forecasting benchmarks~\cite{gifteval,fev,wang2025aries}, the QUALS corpus is constructed exclusively using GIFT-EVAL pre-training data~(231B) and large-scale synthetic series~(8B).

This paper makes the following contributions:

\begin{itemize}[leftmargin=*, nosep]
    \item We explicitly identify the dual imbalance of pattern distribution and learnability that restricts zero-shot forecasting capabilities. 
    \item  We propose a scalable data-driven pipeline to discretize heterogeneous temporal patterns, effectively addressing the extreme long-tail distribution in raw corpora.
    \item We introduce a learnability synchronization mechanism that adaptively recalibrates sampling weights to align learning progress and bridge the overfitting--underfitting gap across patterns.
    \item Extensive benchmarks demonstrate that QUALS delivers consistent zero-shot gains, achieving superior accuracy under strict leakage-free evaluation with substantially reduced training budgets and preprocessing costs.
\end{itemize}

Section 2 reviews related work. Section 3 covers preliminaries. Section 4 details the proposed QUALS. Section 5 reports on the experimental study.  Section 6  visualizes and analyzes each stage of QUALS; and Section 7 concludes.



==> sections/introduction_v1.tex <==
\section{Introduction}

Time series data are pervasive in large-scale critical infrastructures such as transportation management~\cite{}, cloud resource monitoring~\cite{}, and public safety systems~\cite{}. Given the inherent heterogeneity~\cite{BasicTS, TFB} of these application scenarios, building universal time series forecasting models that can transfer across domains and generalize in a zero-shot manner has become a central challenge for both academia~\cite{TimeMoE, Sundial} and industry~\cite{Chronos-2, MOIRAI-2}. Achieving this goal requires not only strong representation capacity, but more importantly, an effective way to manage the dramatic distribution shifts across heterogeneous domains.

Inspired by recent advances in Natural Language Processing (NLP) \cite{GPT, LLaMA, QWen}, universal time series forecasting has largely relied on training large-scale models over massive corpora to induce the emergence of zero-shot forecasting ability. Representative models such as Chronos~\cite{Chronos-1}, MOIRAI~\cite{MOIRAI-1}, and Sundial~\cite{Sundial} all perform large-scale pre-training based on different Transformer architectures and have achieved state-of-the-art performance. However, unlike NLP, where progress has been driven primarily by scaling model parameters, universal time series forecasting has relied more heavily on scaling data volume. To cope with the extreme heterogeneity of cross-domain data and improve zero-shot performance, existing studies tend to indiscriminately aggregate open-source datasets from diverse domains and continuously expand corpus size, as illustrated in Figure 1(a). For example, the above three models contain only 710M, 311M, and 444M parameters, respectively, while their corresponding training corpora reach 84B, 231B, and even 1032B points.
% These works collectively highlight the strong dependence of current emergent zero-shot capability on data scale.
Although this brute-force data accumulation paradigm brings certain generalization gains, it not only causes substantial computational waste~\cite{BLAST}, but also dramatically exacerbates the difficulty of managing data distributions.

In fact, the root cause of the current \textit{data inefficiency} lies in the excessive emphasis on sheer data volume while neglecting a principled characterization of the underlying \textit{data diversity}. Specifically, the training corpora of existing universal forecasting models suffer from two core challenges. \textit{First, the data distribution is severely imbalanced.} Expanding source domains does not naturally guarantee diversity in intrinsic temporal patterns. For instance, the left side of Figure 1(b) shows that climate data account for as much as 87\% of the GIFTEvalPretrain~\cite{GIFT_Eval} corpus, while the deep representation visualization on the right further confirms the extreme skewness of the distribution. Under such a long-tailed distribution, simple sampling strategies~\cite{naive sampling and stratified sampling studies} cause the model to overfit frequent patterns while underfitting rare ones. \textit{Second, heterogeneous patterns exhibit substantially different learnability}. Time series vary greatly in complexity: simple and clean motifs are easily captured by neural models, whereas complex patterns involving multiple periodicities or strong non-stationarity pose much greater optimization difficulty. Figure 1(c) shows that Chronos~\cite{Chronos} converges at dramatically different speeds over different pattern types (each line).

Therefore, managing the training data distribution from a diversity-oriented perspective is the key to improving data efficiency and preventing training budgets from growing without bound. Unfortunately, existing studies have paid little attention to the equilibrium of universal time series corpora. Although recent work such as BLAST~\cite{BLAST} attempts to alleviate data imbalance using heuristic statistical features, these shallow ones neither capture deep temporal semantics accurately nor scale efficiently due to their high computational cost. More importantly, they completely ignore the intrinsic disparity in learnability across different data patterns.


\begin{figure}[t]
  \centering
  \includegraphics[width=0.95\linewidth]{figures/intro2.pdf}
  \vspace{-5pt}
  \caption{Overview of existing corpus curation paradigms and their inherent flaws in pattern distribution and learnability imbalances.}
  \vspace{-5pt}
  \label{fig:intro}
\end{figure}


To break through this data bottleneck, we propose QUALS, a pattern quantization and learnability synchronization framework. As shown in Table 1, unlike prior approaches that either rely on brute-force data accumulation or expensive heuristic descriptors, QUALS establishes a new pre-training corpus sampling paradigm with dual equilibrium, aiming to simultaneously align pattern distribution and learnability.

First, to overcome the shallow representation limitations and computational overhead of heuristic features, QUALS introduces a fully data-driven mechanism for pattern discretization and binning. Specifically, by combining a multi-scale quantization architecture with a spectrum-aware strategy, we map highly heterogeneous time series into a discrete pattern space and partition them into uniform pattern bins. This process not only effectively disentangles complex temporal characteristics at low computational cost, but also corrects the severe long-tail distribution in the raw corpus, ensuring that rare yet critical patterns are no longer overwhelmed during sampling.

Second, to address the substantial discrepancy in convergence difficulty across temporal patterns, QUALS further introduces a learnability synchronization mechanism. Built upon an offline Group Relative Policy Optimization (GRPO) strategy, this mechanism dynamically evaluates the convergence speed of each pattern bin during proxy training and adaptively recalibrates sampling weights accordingly. By prioritizing difficult patterns while moderately suppressing easy ones, QUALS enforces synchronized learning progress across the entire corpus, effectively bridging the overfitting–underfitting gap between heterogeneous patterns.

Overall, by enforcing this dual equilibrium over large-scale corpora, QUALS substantially reduces redundancy during pre-training. This not only greatly improves data utilization efficiency, but also significantly cuts pre-training cost. For example, {\color{red}[insert the most visually striking experimental result here.]}

% \begin{table}[t]
%   \centering
%   \caption{Comparison of different corpus curation paradigms.}
%   \vspace{-5pt}
%   \label{tab:comparison}
%   \resizebox{\linewidth}{!}{%
%   \begin{tabular}{lccc}
%     \toprule[1.2pt]
%     \multirow{2}{*}{\textbf{Challenges}} & \multirow{2}{*}{\textbf{QUALS (Ours)}} & \textbf{BLAST} & \textbf{Others} \\
%     &  & \cite{shao2025blast} & \cite{ansari2024chronos,woo2024moirai,shi2024timemoe,liu2024timer} \\
%     \midrule
%     \begin{tabular}[c]\textbf{Distribution}\\\textbf{Imbalance}\end{tabular}
%     & Deep Data-Driven & Heuristic & Naive/Stratified \\
%     \midrule
%     \begin{tabular}[c]{@{}c@{}}\textbf{Learnability}\\\textbf{Synchronization}\end{tabular}
%     & GRPO-Synchronized & $\times$ & $\times$ \\
%     \bottomrule[1.2pt]
%   \end{tabular}%
%   }
% \end{table}

\begin{table}[]
  \centering
  \caption{Comparison of different corpus curation paradigms.}
  \label{tab:comparison}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|c}
\toprule[1.2pt]
\textbf{Challenges} & \begin{tabular}[c]{@{}c@{}}\textbf{QUALS}\\ \textbf{(Ours)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{BLAST}\\ 
{~\cite{shao2025blast}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Others}\\ {\cite{ansari2024chronos,woo2024moirai,shi2024timemoe,liu2024timer}}\end{tabular} \\

\midrule

\begin{tabular}[c]{@{}c@{}}Distribution\\ Imbalance\end{tabular}& Deep Data-Driven  & Heuristic & Naive/Stratified \\
\midrule
\begin{tabular}[c]{@{}c@{}}Learnability\\ Synchronization\end{tabular} & GRPO-Synchronized  & $\times$ & $\times$ \\
\bottomrule[1.2pt]
\end{tabular}
}
\end{table}



% \begin{table}[t]
%   \centering
%   \caption{Comparison of different corpus curation paradigms.}
%   \vspace{-5pt}
%   \label{tab:comparison}
%   \resizebox{\linewidth}{!}{%
%   \begin{tabular}{lccc}
%     \toprule
%     & \multirow{2}{*}{\textbf{QUALS (Ours)}} & \textbf{BLAST} & \textbf{Others} \\
%     &  & \cite{shao2025blast} & \cite{ansari2024chronos,woo2024moirai,shi2024timemoe,liu2024timer} \\
%     \midrule
%     \textbf{Distribution Imbalance} & Deep Data-Driven & Heuristic & Naive/Stratified \\
%     \textbf{Learnability Synchronization} & GRPO-Synchronized & $\times$ & $\times$ \\
%     \bottomrule
%   \end{tabular}%
%   }
% \end{table}


The main contributions of this paper are summarized as follows:
\begin{itemize}
    \item We are the first to systematically reveal the dilemma of dual imbalance in universal time series pre-training corpora, namely pattern distribution skewness and learnability discrepancy, and we propose the QUALS framework to provide a new perspective on efficient cross-domain corpus management.
    \item We propose a fully data-driven and highly scalable method for temporal pattern disentanglement, replacing expensive handcrafted heuristic features with a lower-cost alternative and effectively addressing the long-tail issue in large-scale time series data.
    \item We design a GRPO-based learnability synchronization mechanism that adaptively balances optimization difficulty across heterogeneous patterns without manual intervention, thereby fundamentally mitigating the underfitting/overfitting problem caused by data skew.
    \item Extensive experiments show that QUALS significantly improves the data efficiency of universal time series models, achieving more accurate and stable zero-shot forecasting performance while greatly reducing both training budget and pre-processing cost. 
\end{itemize}


Section 2 reviews related work. Section 3 covers preliminaries. Section 4 details the proposed QUALS. Section 5 reports on the experimental study.  Section 6  visualizes and analyzes each stage of QUALS; and Section 7 concludes.



==> sections/related_work.tex <==
\section{Related Work}
\label{sec:rw}
\subsection{Universal Time Series Forecasting}
Universal time series forecasting~\cite{li2025tsfm} aims to build foundation models with robust zero-shot generalization across unseen domains. The fundamental paradigm relies on training advanced neural architectures over massive datasets to induce these zero-shot capabilities.

Mainstream models predominantly adopt Transformer architectures across three paradigms: \textit{encoder-only} models learning transferable representations via masked modeling or reconstruction  \cite{MOMENT,liu2024moiraimoe,woo2024moirai, wang2025towards}; \textit{decoder-only} models treating forecasting as conditional autoregressive generation \cite{TimesFM,shi2024timemoe,liu2024timer,DBLP:journals/corr/abs-2511-11698,TimeXL}; and \textit{encoder-decoder} models using series discretization to frame probabilistic forecasting as sequence-to-sequence tasks  \cite{Chronos, ansari2025chronos2, DBLP:conf/icml/0004Q00RP0G25}. Complementary works explore alternative inductive biases, including prior-based meta-forecasting and cross-modal transfer  \cite{DAM,ForecastPFN,TTM,DBLP:conf/icml/ChenS0WSL25}

Despite these architectural divergences, the consensus is that the emergence of zero-shot capabilities is fundamentally driven by data rather than mere structural design. Consequently, a prevalent trend in current research is to blindly scale up training pipelines by aggregating massive, multi-domain corpora to enhance performance. However, this unchecked data scaling exposes critical vulnerabilities in data distribution and utilization efficiency, necessitating a closer examination of pre-training corpora

\subsection{Time Series Pre-training Corpora}
Time-series corpora constitute the core foundation of universal forecasting capability. Existing studies predominantly follow a scale-driven paradigm, aggregating massive real-world datasets to maximize distributional coverage. \rev{Representative examples include LOTSA~(231B) for MOIRAI~\cite{woo2024moirai}, the Chronos corpus~(84B)~\cite{Chronos}, the Time-300B corpus for TimeMoE~\cite{shi2024timemoe}, and UTSD for Timer~\cite{liu2024timer}. When training exposure follows source proportions or concentrates on repetitive motifs, rare but informative patterns remain underrepresented, wasting budget and limiting zero-shot generalization---a problem that persists under naive sampling and is only partially alleviated by coarser balancing schemes.}

\rev{To mitigate such exposure imbalance, subsequent work explores progressively finer balancing strategies.
\textit{Dataset-level balancing} assigns comparable training exposure across source datasets; MOIRAI~\cite{woo2024moirai} implements capped dataset-level stratification on LOTSA, and Chronos~\cite{Chronos} adopts dataset-uniform training over its pre-training corpus.
\textit{Domain-level balancing} further controls exposure across semantic domains; Timer~\cite{liu2024timer} constructs UTSD with approximately balanced domain scale before training.
\textit{Pattern-level balancing} moves to temporal motifs themselves: BLAST~\cite{shao2025blast} partitions the corpus using handcrafted statistical descriptors, and catch22~\cite{lubba2019catch22} offers a lighter feature-based bucketing alternative.
These strategies reduce redundancy from over-exposing dominant patterns, yet they still face fundamental limitations:}
\begin{itemize}[leftmargin=*, nosep]
\item \textit{Pattern Distribution.} \rev{Dataset- and domain-level balancing remain coarse-grained: multiple datasets from the same domain can still accumulate high exposure, and dominant motifs within a domain may persist. Heuristic pattern bucketing partially addresses this, but shallow features are costly at scale and may miss deep temporal semantics~\cite{shao2025blast}.}
\item \textit{Pattern Learnability.} Equal sampling priority across heterogeneous patterns overlooks differences in optimization difficulty~\cite{cheng2023weakly}. Since models learn simple motifs much faster than complex ones~\cite{wang2025aries, qiu2025easytime}, such uniform treatment leads to optimization misalignment, where easy patterns dominate gradient updates while difficult ones remain under-optimized.
\end{itemize}

\begin{table}[t]
  \centering
  \setlength{\abovecaptionskip}{0.cm}
  \setlength{\belowcaptionskip}{0.cm}
    \renewcommand\arraystretch{1}
  \caption{\rev{Comparison of corpus curation paradigms. ``Others'' denotes scale-driven corpora with naive sampling or dataset-/domain-/pattern-level balancing~\cite{Chronos,woo2024moirai,shi2024timemoe,liu2024timer,shao2025blast}.}}
\label{tab:comparison}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|c}
\toprule[1.2pt]
\textbf{Challenges} & \begin{tabular}[c]{@{}c@{}}\textbf{QUALS}\\ \textbf{(Ours)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{BLAST}\\ 
{~\cite{shao2025blast}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Others}\\ {\cite{Chronos,woo2024moirai,shi2024timemoe,liu2024timer}}\end{tabular} \\
\midrule
\begin{tabular}[c]{@{}c@{}}Distribution\\ Imbalance\end{tabular}& Deep Data-Driven  & Heuristic & \rev{Dataset/Domain/Pattern-level} \\
\midrule
\begin{tabular}[c]{@{}c@{}}Learnability\\ Synchronization\end{tabular} & GRPO-Synchronized  & $\times$ & $\times$ \\
\bottomrule[1.2pt]
\end{tabular}
}

\end{table}

As shown in Table~\ref{tab:comparison}, existing corpus construction paradigms remain scale-centric, and even recent balancing efforts do not jointly address pattern distribution and learnability in a systematic way. As a result, data efficiency remains suboptimal and complex data distributions remain poorly managed. Therefore, how to systematically distill, compress, and organize massive time-series data to better unlock the potential of large-scale pre-training remains a key challenge for universal forecasting. To tackle this challenge, QUALS provides a unified corpus curation paradigm that combines deep data-driven pattern organization with GRPO-synchronized learnability-aware curation.



==> sections/response_general_g1_g2_g3.tex <==
% !TeX root = ../main.tex
We thank the meta-reviewer and all reviewers for their constructive feedback and revision recommendations.
Below we summarize our responses to the overlapping concerns raised by the Associate Editor (AE) and Reviewers~\#1--\#3:
\textbf{(G1) related work and positioning},
\textbf{(G2) expanded comparisons and controlled evaluation}, and
\textbf{(G3) the design rationale and necessity of the three-stage framework}.
Detailed point-by-point replies follow in the reviewer-specific sections; all corresponding changes are highlighted in the revised manuscript.

\resptitle{Response G1: Related Work and Positioning.}
To address the reviewers’ concerns regarding the scope and novelty of QUALS, we revised Section 2, especially Section 2.2, along three dimensions: we clarified the data-centric scope of the work, reorganized prior corpus-construction approaches according to the granularity of data-exposure control, and more explicitly distinguished QUALS from existing pattern-level corpus-curation methods. We also added TSFM-Bench [7] as a relevant evaluation framework. The corresponding revisions are summarized below.

% {\color{red}\respblock{Related-work clarification.} We revised Section~\ref{sec:rw}, especially Section~2.2, to clarify the positioning of QUALS relative to prior TSFM corpus-construction approaches and the evaluation framework introduced by TSFM-Bench~\cite{li2025tsfm}.

\respblock{Response G1.1: Data-Centric Scope.}
QUALS is a data-centric framework for constructing and sampling pre-training corpora rather than a new forecasting architecture. It leaves the underlying model architecture unchanged and evaluates whether improved corpus construction can further enhance existing universal forecasting models. This distinction clarifies the relationship between QUALS and model-centric approaches such as Chronos~\cite{Chronos}, TimeMoE~\cite{shi2024timemoe}, and MOIRAI~\cite{woo2024moirai}.

\respblock{Response G1.2: Granularity-Based Taxonomy of Corpus Construction.}
We reorganized Section 2.2 according to the granularity at which pre-training data exposure is controlled. Scale-driven pipelines aggregate increasingly large corpora but may repeatedly expose models to dominant temporal motifs. Dataset- and domain-level strategies control exposure using source metadata, whereas more fine-grained approaches, such as BLAST~\cite{shao2025blast} and Catch22-based feature bucketing~\cite{lubba2019catch22}, operate at the pattern level. Table~\ref{tab:comparison} summarizes these distinctions and shows that existing strategies differ in both the granularity of corpus control and the information used to guide sampling.

\respblock{Response G1.3: Positioning of QUALS.}
Existing pattern-level corpus-curation approaches primarily rely on handcrafted statistical descriptors and focus on balancing pattern exposure. In contrast, QUALS learns a discrete pattern space from deep temporal representations and further adjusts corpus sampling according to pattern-specific convergence behavior. {\textit{It therefore jointly addresses pattern-distribution imbalance and heterogeneous learnability.}} The corresponding empirical comparisons with dataset-, domain-, and pattern-level alternatives are reported in Table~\ref{tab:vldb_all_benchmarks_sampling_tsfm_last} and summarized in Response G2.

\resptitle{Response G2: Expanded Comparisons and Controlled Evaluation.}
To address the reviewers’ concerns regarding missing corpus-construction baselines, evaluation breadth, and comparison fairness, we revised the experimental evaluation along four dimensions: comparison scope, retraining protocol, benchmark coverage, and empirical analysis. The corresponding revisions and findings are summarized below.

\respblock{Response G2.1: Expanded Comparison Scope.}
In response to R1:W2, R2:W1, and the AE’s revision request, we added data-selection and corpus-construction baselines to Table~\ref{tab:vldb_all_benchmarks_sampling_tsfm_last} and evaluated them alongside QUALS. 
Specifically, we conducted new pre-training runs for ChronosBolt~\cite{Chronos} and TimeMoE~\cite{shi2024timemoe} under the evaluated corpus-construction strategies, while retaining their official checkpoints as references:

\begin{itemize}[leftmargin=*, nosep]
\item \textit{Original}: official checkpoints under their originally reported pre-training settings.
\item \textit{AvgDataset}: uniform exposure across GIFT-Eval Pretrain sub-datasets~\cite{gifteval}.
\item \textit{AvgDomain}: uniform exposure across the domain labels in GIFT-Eval Pretrain~\cite{gifteval}.
\item \textit{Catch22}: Catch22-based feature bucketing within the BLAST-style corpus-balancing pipeline~\cite{lubba2019catch22, shao2025blast}.
\item \textit{BLAST}: pattern-level corpus balancing based on statistical descriptors~\cite{shao2025blast}.
\item \textit{Online-GRPO}: an online alternative that updates sampling weights during model pre-training on the QUALS candidate corpus.
\item \textit{QUALS}: our full pipeline combining pattern-level corpus balancing with learnability synchronization.
\end{itemize}

\respblock{Response G2.2: Controlled Retraining Protocol.}
All retrained variants use the same GIFT-Eval Pretrain source data~\cite{gifteval} and preserve the architecture and model-specific training and evaluation settings within each model family. The principal controlled factor is the corpus-construction and sampling strategy. Table~\ref{tab:response_token_budget} reports the pre-training token budgets of all variants.

\respblock{Response G2.3: Broader Evaluation Coverage.}
We additionally report the complete TSFM-Bench results~\cite{li2025tsfm} in Table~\ref{tab:tsfm}.
Because TSFM-Bench originally reports per-dataset performance and space is limited, we follow the conventions used in GIFT-Eval~\cite{gifteval} and FEV~\cite{shchur2025fev} and convert model performance into skill scores relative to a Seasonal Naive baseline~\cite{makridakis2020m4}.
% 
Furthermore, we also compare QUALS-pretrained models with recent and classical domain-specific forecasting models in Table~\ref{domain_specific}.

\respblock{Response G2.4: Main Empirical Findings.} QUALS achieves the strongest overall performance across the two model families while using substantially smaller pre-training budgets than several alternative corpus strategies.
% 
For ChronosBolt$_s$, QUALS reduces the GIFT-Eval-B average MASE from 0.736 for Original and 0.684 for BLAST to 0.663.
% 
For TimeMoE$_b$, it reduces the corresponding MASE from 0.888 and 0.760 to 0.734.
% 
Dataset- and domain-level balancing, handcrafted feature bucketing, and online policy updating may be competitive on individual datasets or metrics, but none matches QUALS consistently across the full evaluation suite.

\input{tables/response_token_budget}
\input{tables/comparison}


\resptitle{Response G3: Design Rationale and Necessity of the Three-Stage Framework.}

To address the reviewers’ concerns about the rationale and necessity of the three-stage design, we revised Section 3 to formally define learnability and reorganized Section 4 around two complementary objectives: \textit{pattern equilibrium}, implemented by Stages 1–2, and \textit{learnability equilibrium}, implemented by Stage 3. The three stages therefore address distinct constraints in large-scale corpus construction rather than forming an arbitrary sequence of interchangeable modules.


\respblock{Response G3.1: Design Decomposition and Motivation.}
Universal forecasting depends not only on corpus scale but also on balanced training exposure. Repeatedly sampling dominant motifs wastes computation and underexposes rare patterns. We therefore decompose corpus equilibrium into two objectives.

\textit{Pattern equilibrium} seeks balanced exposure across heterogeneous temporal morphologies and requires a countable pattern space for controlled sampling. \textit{Learnability equilibrium} further accounts for the fact that equally represented patterns may converge at different rates and therefore require different training budgets. Stages 1–2 address the former, while Stage 3 addresses the latter.


\respblock{Response G3.2: Pattern Equilibrium and the Necessity of Stages 1–2.}
Existing pipelines do not fully achieve pattern equilibrium. Scale-driven aggregation produces heavy-tailed distributions over datasets and motifs. Dataset- or domain-level balancing controls source labels rather than temporal morphology, while BLAST~\cite{shao2025blast} and Catch22-based alternatives~\cite{lubba2019catch22} provide finer-grained control but remain limited by handcrafted descriptors and large-scale computational cost.

Stage 1 maps raw, variable-length series into countable temporal units through multi-scale patch splitting and fixed-codebook vector quantization~\cite{DBLP:conf/iccv/LiuL00W0LG21,DBLP:conf/nips/OordVK17}. Anti-collapse training promotes stable codebook utilization and coverage of diverse temporal patterns.

However, patch-level activations still inherit the frequency bias of the original corpus and do not directly define balanced series-level sampling units. Stage 2 therefore aggregates patch representations into series-level embeddings and applies PCA- and ECDF-based binning to construct a finite pattern space $\mathcal{U}$ with more uniform occupancy.

We then uniformly resample GIFT-Eval Pretrain~\cite{gifteval} in $\mathcal{U}$ to form the candidate corpus $\mathcal{R} \in \mathbb{R}^{N \times L}$, where $N{=}20$M and $L{=}4096$. Although subsequent sampling could operate directly on the raw corpus, materializing $\mathcal{R}$ avoids repeated online bin lookup, unifies storage formats, and enables efficient chunked I/O. Table~\ref{tab:vldb_all_benchmarks_sampling_tsfm_last} evaluates handcrafted alternatives such as Catch22 and BLAST, while Table~\ref{tab:ablation_transposed_quals_321_best} reports the Stage 1 and Stage 2 ablations.


\respblock{Response G3.3: Learnability Equilibrium and the Necessity of Stage 3.}
Equal pattern counts do not guarantee equal optimization progress. Different patterns may require different training budgets because of temporal dependence, morphological complexity, and signal-to-noise ratio. We define the learnability of bin $u_i$ as the effective budget needed to reach a convergence level:
\begin{equation}
B_i^\star=\min\{B:\ell_i(B)\le \tau_i\},
\end{equation}
where $\ell_i(B)$ is the validation loss after budget $B$, and $\tau_i$ is a bin-specific threshold.
A smaller $B_i^\star$ indicates easier learnability, while a larger $B_i^\star$ indicates a harder pattern.

In large-scale universal forecasting, however, $B_i^\star$ is not directly observable: the total budget is fixed, each bin cannot be trained independently to convergence, and the proper threshold $\tau_i$ is unknown. We therefore use an observable proxy based on uniform probing. Under uniform exposure, the convergence speed of bin $u_i$ at training stage $t$ is measured as
\[
r_{i,t}=-\frac{\Delta \ell_i(t)}{\Delta t}.
\]
The resulting learnability profile is $\mathbf{R}\in\mathbb{R}^{M\times T}$, where larger $r_{i,t}$ indicates faster learning under equal exposure. Learnability equilibrium then seeks sampling weights $w_i$ such that the effective learning progress $p_{i,t}=w_i r_{i,t}$ is synchronized across bins under the same total budget.

This is a noisy stochastic allocation problem: the candidate corpus contains $M=2499$ valid bins, mini-batches observe only a subset of each bin, and bin-wise progress is coupled through shared parameters. A direct rule such as $w_i\propto 1/r_i$ is therefore unstable.

Stage 3 uses an offline two-phase procedure. First, a proxy model is trained on $\mathcal{R}$ with uniform bin weights, and bin-wise convergence speeds are recorded. Second, with the learnability profile fixed, a policy $\pi_{\theta}$ maps each bin embedding $v_i$ to a weight $w_i$.
% 
GRPO~\cite{fu2025reward} optimizes the synchronization reward
\begin{equation}
R_{i,t}=-(w_i r_{i,t}-\bar{p}_t)^2,\quad
\bar{p}_t=\frac{1}{|\mathcal{B}|}\sum_{j\in\mathcal{B}}w_j r_{j,t}.
\end{equation}
The reward assigns greater exposure to slow-learning bins and less exposure to fast-learning bins. The final weight vector $\mathbf{w}^*$ is then fixed for corpus resampling and final model pre-training.

\respblock{Response G3.4: Offline Design versus Online Weight Updating.}
QUALS decouples GRPO optimization from forecasting-model training. This avoids repeated model retraining during policy search and prevents unstable intermediate weights from perturbing proxy-model optimization.

The Online-GRPO baseline instead updates sampling weights during proxy pre-training. Although simpler, it is more sensitive to transient training states and performs less consistently in Table II. We also tested a fully coupled variant that fed intermediate GRPO weights back into proxy training in real time. Its reward estimates and sampling weights remained unstable, preventing the proxy model from converging.

QUALS  adopts offline profiling, offline GRPO, and fixed-weight resampling. Together with the ablations in Table~\ref{tab:ablation_transposed_quals_321_best} and the Online-GRPO comparison in Table~\ref{tab:vldb_all_benchmarks_sampling_tsfm_last}, these results support both the two-objective decomposition and the role of each stage.


==> sections/response_letter.tex <==
% !TeX root = ../main.tex
\pagenumbering{roman}
\setcounter{table}{0}
\setcounter{figure}{0}
\renewcommand{\thetable}{\Roman{table}}
\renewcommand{\thefigure}{\Roman{figure}}
\renewcommand{\theHtable}{response.table.\Roman{table}}
\renewcommand{\theHfigure}{response.figure.\Roman{figure}}
\twocolumn[
\begin{center}
{\fontsize{16pt}{19pt}\selectfont\bfseries Response Letter for Submission 59\par}
{\fontsize{14pt}{17pt}\selectfont\bfseries ``QUALS: Corpus Equilibrium for Universal Forecasting via Pattern Quantization and Learnability Synchronization''\par}
% \vspace{10pt}
{\fontsize{11pt}{13pt}\selectfont
Yujie Li$^{1,2}$, Zezhi Shao$^{1\ast}$, Chengqing Yu$^{1,2}$, Yisong Fu$^{1,2}$, Weijie Zhu$^{1}$, Yifan Du$^{1}$, Jilin Hu$^{3}$, Bin Yang$^{3}$, \\Yongjun Xu$^{1,2}$, Fei Wang$^{1,2\ast}$\par}
{\normalsize
$^{1}$State Key Laboratory of AI Safety, Institute of Computing Technology, Chinese Academy of Sciences, Beijing, China\par
$^{2}$University of Chinese Academy of Sciences, Beijing, China\par
$^{3}$School of Data Science and Engineering, East China Normal University, Shanghai, China\par}
{\normalsize
\{liyujie23s, shaozezhi, yuchengqing22b, fuyisong24s, zhuweijie26s, duyifan, xyj, wangfei\}@ict.ac.cn,
\{jlhu, byang\}@dase.ecnu.edu.cn\par}
\end{center}
]
\vspace{10pt}
\thispagestyle{plain}

\noindent Dear PVLDB chairs, meta-reviewer, and reviewers,
\vspace{10pt}

Thank you very much for your valuable comments and suggestions. We have carefully revised the manuscript and addressed the issues raised in the reviews. In the following, we summarize the major revisions and provide detailed responses to the comments. In addition to the responses to each reviewer and the meta-reviewer, we add a general response section that provides an overview of the responses to important and general issues.
We hope that the reviewers would read this section first.
We use ``R'' to denote ``Reviewer'', ``W'' to denote ``Weakness'', ``D'' to denote ``Detailed Comment'', ``A'' to denote ``Response'', and ``G" to denote ``General Response". We have also highlighted the revised parts in our manuscript.

\vspace{10pt}
\noindent Yours sincerely,\\
Yujie, Zezhi, Chengqing, Yisong, Weijie, Yifan, Jilin, Bin, Yongjun, and Fei.

\section*{General Response}
\vspace{4pt}


\input{sections/response_general_g1_g2_g3}

% \vspace{10pt}
\section*{Meta-Reviewer}

\noindent \respblock{Issue AE.1:} \textit{Expand related work.}

\noindent \textbf{Response AE.1:} 
Thank you for highlighting this important revision item.
% 
We revised Section 2, especially Section 2.2, to clarify the data-centric scope of QUALS, reorganize prior corpus-construction approaches according to the granularity of data-exposure control, and more explicitly distinguish QUALS from existing pattern-level corpus-curation methods. We also added TSFM-Bench~\cite{li2025tsfm} as a relevant evaluation framework. These revisions are summarized in Responses G1.1–G1.3.

\noindent \respblock{Issue AE.2: } \textit{Add relevant baselines in the experiments.}

\noindent \textbf{Response AE.2:} 
We added controlled comparisons covering dataset-level, domain-level, handcrafted-feature-based, statistical pattern-level, and online weighting strategies.
% 
We conducted new pre-training runs for ChronosBolt~\cite{Chronos} and TimeMoE~\cite{shi2024timemoe} under these corpus-construction strategies, while retaining their official checkpoints as references. We also broadened the evaluation with TSFM-Bench~\cite{li2025tsfm} and comparisons against domain-specific forecasting models. The revised experimental design and findings are summarized in Responses G2.1–G2.4 and reported in Tables I–IV.

\noindent \respblock{Issue AE.3:} \textit{Strengthen the justification of design decisions.}

\noindent \textbf{Response AE.3:} 
We revised Sections 3 and 4 to formalize learnability and reorganize the design rationale around two complementary objectives: pattern equilibrium, implemented by Stages 1–2, and learnability equilibrium, implemented by Stage 3.
% 
We further explain why QUALS adopts offline profiling and optimization rather than simpler online alternatives, with supporting comparisons and ablations in Tables~\ref{tab:vldb_all_benchmarks_sampling_tsfm_last} and \ref{tab:ablation_transposed_quals_321_best}. These revisions are summarized in Responses G3.1–G3.4.



\input{tables/domain_specific}
\input{tables/tsfm_bench}

\section*{Reviewer \#1}

\noindent \respblock{Issue Q1.1 (W1):} \textit{The technical contribution of this paper is somewhat unclear. The overall three-stage framework can be implemented in different ways. For example, the first stage can be replaced by other representation learning methods, the second stage can be implemented using different clustering approaches, and the third stage can also be achieved without reinforcement learning. The overall data selection logic is relatively straightforward, and it is not clear what the necessity is for the specific three-stage design proposed by the authors.}

\noindent \textbf{Response A1.1:} 
Thank you for the valuable comment. We agree that the original manuscript did not sufficiently explain why the three stages are necessary, and we revised Sections~\ref{sec:preliminaries} and~\ref{sec:method} accordingly. The key point is that QUALS is not an arbitrary combination of three modules. It decomposes corpus equilibrium into two distinct objectives: pattern equilibrium, implemented by the construction policy $\pi_c$, and learnability equilibrium, implemented by the sampling policy $\pi_s$.

Stages~1--2 implement $\pi_c$ because pattern balancing first requires a countable temporal pattern space and then a balanced series-level corpus.
%
In Stage~1, VQ-SwinTTS uses patch splitting to support variable-length time series, multi-scale encoding to capture patterns at different temporal resolutions, and reconstruction learning to preserve temporal information. Shifted-window attention enables scalable representation extraction for large-scale pretrain corpus, while vector quantization and stabilized codebook optimization produce countable pattern identities with stable codebook utilization.
%
Because these architectural components are tightly coupled, exhaustively ablating them one by one would require repeatedly retraining both the Stage~1 model and the downstream universal forecasting models on a large-scale corpus, resulting in prohibitively high computational costs. We therefore conduct three complementary evaluations to validate the effectiveness of the Stage~1 design from different perspectives.
% 
Section~5.6.1 verifies intra-code coherence, inter-code separability, and pattern semantics through similarity analysis and visualization. Table~\ref{tab:vldb_all_benchmarks_sampling_tsfm_last} shows the advantages of the learned representation over the simpler Catch22-~\cite{lubba2019catch22} and BLAST~\cite{shao2025blast}-based alternatives, while the \textit{w/o Stage~1} ablation in Table~\ref{tab:ablation_transposed_quals_321_best} confirms the overall contribution of Stage~1.
% to downstream performance.

Stage~2 is required because Stage~1 achieves meaningful pattern quantization but does not enforce uniformity in the learned codebook space. Figure~\ref{fig:codebook_analysis} shows that the Stage~1 codebook has a markedly non-uniform information distribution across latent dimensions, and therefore cannot be directly treated as a balanced sampling space. Stage~2 applies PCA to decorrelate the latent dimensions and identify their relative information content, allocates more partitions to informative dimensions, and uses ECDF-based boundaries to construct finite series-level bins with more balanced occupancy. Removing this stage also leads to weaker performance as shown in Table~\ref{tab:ablation_transposed_quals_321_best}.

Stage~3 implements $\pi_s$ because uniform pattern counts do not imply uniform optimization progress. QUALS therefore profiles bin-wise convergence and derives sampling weights to synchronize learning progress across patterns with heterogeneous learnability. Removing learnability synchronization or replacing it with online policy updating performs worse, as shown in Table~\ref{tab:ablation_transposed_quals_321_best} and the \textit{Online-GRPO} comparison in Table~\ref{tab:vldb_all_benchmarks_sampling_tsfm_last}.

We therefore revised the manuscript to present the three stages as responses to distinct design constraints rather than as interchangeable pipeline components. Stage~1 constructs scalable and countable temporal representations, Stage~2 organizes them into a balanced series-level pattern space, and Stage~3 allocates the training budget according to heterogeneous pattern learnability. The complete rationale and supporting evidence are summarized in Responses~G3.1--G3.4.


\noindent \respblock{Issue Q1.2 (W2):} \textit{The paper lacks some important baseline comparisons and discussion of related work on data selection. The number of data selection methods included for comparison is limited. For example, it is unclear how a simple strategy such as randomly sampling the same proportion of data from different sub-dataset domains would perform. In addition, many data selection methods from other domains could likely be applied directly, which makes it difficult to demonstrate the necessity and uniqueness of the proposed approach.}

\noindent \textbf{Response A1.2:} 
We reorganized the related-work discussion in Section~\ref{sec:rw} and added controlled corpus-construction comparisons in Table~\ref{tab:vldb_all_benchmarks_sampling_tsfm_last}.
% 
The requested source-level controls are represented by \textit{AvgDataset} and \textit{AvgDomain}, which impose uniform exposure across GIFT-Eval Pretrain~\cite{gifteval} sub-datasets or domain labels. We further include \textit{Catch22}~\cite{lubba2019catch22} as a handcrafted-feature bucketing baseline, \textit{BLAST}~\cite{shao2025blast} as a statistical pattern-level balancing baseline, and \textit{Online-GRPO} as an online weighting alternative.

These baselines cover the principal design dimensions relevant to large-scale time-series corpus construction, including source granularity, pattern representation, and static versus online weighting. All newly retrained variants use the same source data and preserve the model-specific training and evaluation settings within each model family; the \textit{Original} checkpoints are retained separately as official references under their originally reported pre-training settings. See Responses G1.2–G1.3 and G2.1–G2.2.

\noindent \respblock{Issue Q1.3 (W3):} \textit{Some details in the method and experimental sections are described vaguely, making it difficult to assess the effectiveness of the proposed design. For instance, what do the learned weights in the third stage look like? In the ablation study of the second stage, is the random sampling of 8000 samples still retained? What is the impact of different sampling ratios?}

\noindent \textbf{Response A1.3:}
Thank you for pointing out these unclear details. We clarified them in Section~\ref{sec:method}. 
% 
First, the learned weights in Stage~3 form a normalized bin-level vector $\mathbf{w}^*\in\mathbb{R}^{M}$ over the 2,499 valid pattern bins, with $\sum_i w_i=1$.
% 
Each entry is the final sampling probability assigned to one pattern bin.
By design, slow-learning bins tend to receive larger probabilities and fast-learning bins smaller ones. Figure~\ref{fig:6in2x3} further visualizes the resulting optimization effect: weighted sampling substantially accelerates the slow-pattern group while changing the already fast-converging group only marginally.

Second, the 8,000-per-bin quota is used to construct the stage 2 candidate corpus of
20M fixed-length series, not the final training probability
% 
The w/o Stage~3 ablation keeps this candidate corpus and uses uniform bin weights, whereas QUALS applies $\mathbf{w}^*$ for learnability-aware resampling.
% 
The w/o Stage 2 ablation instead samples from the 2,048 Stage 1 codebook indices without series-level PCA/ECDF binning.

Third, the 20M candidate-corpus scale was fixed to match the BLAST-level curated scale and retain sufficient within-bin randomness. Stage 3 does not introduce an additional fixed sampling-ratio hyperparameter; it learns the final bin probabilities. We clarified this distinction in the revised manuscript.

We have also released the complete corpus-construction and sampling files at \url{https://huggingface.co/datasets/Blisky-li/QUALS}.

\noindent \respblock{Issue Q1.4 (W4):} \textit{The experiments appear to involve unfair comparisons. The input length used in this paper is 4096, whereas the original baseline papers do not use the same setting. For example, TimeMOE uses four different prediction horizons {96, 192, 336, 720}, with corresponding input time series lengths {512, 1024, 2048, 3072}. However, the results reported with an input length of 4096 seem to achieve nearly identical accuracy. A similar issue exists for Moirai, indicating a noticeable performance reporting gap. In addition, the original Chronos paper is not designed for long-term forecasting, so Sundial may be a more appropriate baseline in this context.}

\noindent \textbf{Response A1.4:}
Thank you for raising the fairness concern. We clarified in Section~\ref{sec:exp} that $L{=}4096$ is the stored corpus-slice length used by QUALS, not a unified evaluation input length.
It is only used to cover the largest supported context; each model still follows its official training and evaluation protocol, including context length, masking, and rollout.
For example, ChronosBolt~\cite{Chronos} uses its 2048-history forecasting setup with 64-step prediction chunks, TimeMoE~\cite{shi2024timemoe} uses its autoregressive 4095-history one-step protocol, and MOIRAI~\cite{woo2024moirai} uses its token-based masking protocol.

Thus, the comparison is controlled within each model family: the architecture and model-specific evaluation protocol are fixed, while the corpus-construction or sampling strategy is varied across the newly retrained variants. The corresponding controls are summarized in Response G2.2.

We agree that Sundial~\cite{liu2025sundial} is a relevant long-horizon architecture. However, comparing against its official checkpoint would conflate architectural and corpus differences, whereas retraining Sundial under every corpus strategy would require a separate set of large-scale experiments beyond the scope of this revision. We therefore focus on representative architectures for which reproducible training pipelines and controlled corpus replacement are available.


\section*{Reviewer \#2}

\noindent \respblock{Issue Q2.1 (W1):} \textit{The authors failed to compare against simpler dataset-level sampling strategies such as weighted dataset sampling.}

\noindent \textbf{Response A2.1:}
Thank you for the suggestion. We added \textit{AvgDataset} and \textit{AvgDomain} as dataset- and domain-level corpus-construction strategies and conducted new pre-training runs for both ChronosBolt and TimeMoE. AvgDataset imposes uniform exposure across source sub-datasets, whereas AvgDomain imposes uniform exposure across domain labels. As reported in Table~\ref{tab:vldb_all_benchmarks_sampling_tsfm_last} and summarized in Responses G2.1–G2.2, both coarse-grained strategies remain weaker than QUALS, despite using larger pre-training token budgets in the reported experiments.

\noindent \respblock{Issue Q2.2 (W2):} \textit{The authors should also better justify the choice of a VQ-SwinTTS codebook over simpler characterization methods. Could similar performance be achieved by using traditional time-series featurization (such as catch22) or component decomposition to bucket the data into patterns?}

\noindent \textbf{Response A2.2:} 
We added Catch22~\cite{lubba2019catch22} as a representative handcrafted-feature bucketing baseline and clarified the rationale for Stages 1–2. This baseline follows the same overall corpus-balancing pipeline as BLAST~\cite{shao2025blast}, but uses catch22 descriptors to define the pattern representation.
% 
We did not introduce a separate STL- or component-decomposition baseline because decomposition alone does not define a complete corpus-construction pipeline: it additionally requires choices regarding period estimation, decomposition configuration, feature aggregation, and binning.
% 
Moreover, such methods primarily expose trend- and seasonality-related structure, whereas Catch22 and BLAST provide broader representative sets of handcrafted temporal descriptors.
% 
Table~\ref{tab:vldb_all_benchmarks_sampling_tsfm_last} shows that the handcrafted alternatives are substantially weaker overall than QUALS, Table~\ref{tab:ablation_transposed_quals_321_best} isolates the contribution of the learned Stage 1 representation, and Table~\ref{tab:quals_blast_efficiency} reports the corresponding large-scale computational comparison. The full rationale is summarized in Response G3.2.


\noindent \respblock{Issue Q2.3 (W3):}  \textit{Similarly for the GRPO-based synchornization. Can we also test simpler alternatives, such as online uncertainty sampling, to demonstrate whether the policy-driven approach is necessary for achieving equilibrium.}

\noindent \textbf{Response A2.3:} We added \textit{Online-GRPO} as an online policy-updating alternative and discuss why QUALS adopts offline profiling plus offline GRPO~\cite{fu2025reward} in General Response~G3. We also examined a simpler uncertainty proxy based on the Stage~1 reconstruction loss, using it to distinguish easy and hard samples. However, this signal did not yield a clear improvement: difficulty in reconstructing historical windows does not necessarily indicate the predictability of future values. Therefore, the revised experiments report \textit{Online-GRPO} as the implemented online alternative, while more forecasting-specific uncertainty sampling remains an interesting direction for future work.

\noindent \respblock{Issue Q2.4 (D1):} \textit{In Figure 1b (right), the legend and axis labels are not very clear. Please discuss the significance of the COV=3.8 value and clarify the specific implications this metric has for the diversity or balance of the corpus.}

\noindent \textbf{Response A2.4:} 
Thank you for pointing this out. We revised both the Introduction and the caption of Figure~\ref{fig:intro}(b) to clarify the data source, visual encoding, axes, and the meaning of COV.

The left pie chart reports domain shares computed from the GIFT-Eval Pretrain metadata. The right panel shows the pattern-bin occupancy distribution obtained using the pattern analysis introduced in this manuscript and projected into two dimensions; the revised caption now explicitly describes the projection and visual encoding.

COV is the coefficient of variation of pattern-bin occupancies, computed as the standard deviation divided by the mean occupancy. A COV of zero would indicate uniform occupancy, whereas COV=3.8 means that the standard deviation is 3.8 times the mean, revealing a highly concentrated and non-uniform pattern distribution. Thus, COV measures corpus imbalance rather than diversity in an abstract sense.



\noindent \respblock{Issue Q2.5 (D2):} \textit{Please expand the explanation of existing SOTA models like TimeMoE or MOIRAI. While these models achieve results through architectural scaling, they do not explicitly address "corpus equilibrium." I am not very sure this is a fair comparison.}

\noindent \textbf{Response A2.5:} 
We clarified the positioning in Responses G1.1 and G1.3. TimeMoE~\cite{shi2024timemoe}, MOIRAI~\cite{woo2024moirai}, and Chronos~\cite{Chronos} are representative model-centric universal forecasters, whereas QUALS is a data-centric framework for corpus construction and sampling.

The revised evaluation contains two complementary types of comparison. The official checkpoints show how QUALS-pretrained models compare with widely used universal forecasters under their originally reported settings. More importantly, the controlled retraining experiments in Responses G2.1–G2.2 keep the architecture and model-specific protocol fixed within each model family and vary the corpus-construction strategy. These within-family comparisons therefore isolate the effect of corpus construction more directly.

\noindent \respblock{Issue Q2.6 (D3):}\textit{ Please explain what "28\% leakage" refers to in this context in Section 5.2.} 

\noindent \textbf{Response A2.6:} The 28\% leakage is measured at the dataset-configuration level in the public FEV-Bench audit~\cite{shchur2025fev}\footnote{\url{https://huggingface.co/spaces/autogluon/fev-bench}}: among the 100 FEV-Bench dataset configurations, 28 appear in the official MOIRAI~\cite{woo2024moirai} pre-training corpus. This gives the official checkpoint a potential memorization advantage on those configurations. Similar overlap is difficult to avoid in early universal forecasting work because both model corpora and benchmarks are often drawn from public time-series datasets.

We clarified this point in Section~5.2. QUALS avoids this issue by constructing its retraining corpus from the open GIFT-Eval Pretrain pool~\cite{gifteval} and excluding benchmark-overlapping sources. Therefore, the QUALS-based retrained models are evaluated under a strictly leakage-free setting, while some official checkpoints retain the declared leakage advantage.



\section*{Reviewer \#3}

\noindent \respblock{Issue Q3.1 (W1, Q1):} \textit{It is not clear why the experimental evaluation solely focuses on zero-shot forecasting or why tsfm-bench [34], which is mentioned early on, is not used for the evaluation. \& The paper argues convincingly the limitations of existing universal forecasting approaches in the Introduction. Why not compare your approach to domain specific models? Why only focus on zero-shot forecasting?}

\noindent \textbf{Response A3.1:} 
Thank you for this important suggestion. We retain zero-shot forecasting as the primary evaluation setting because QUALS targets pre-training corpus construction for universal forecasters, and zero-shot performance directly measures whether corpus construction improves out-of-domain generalization.

We nevertheless broadened the evaluation in two ways. First, Table IV reports TSFM-Bench~\ref{tab:tsfm} skill scores for the QUALS, BLAST, and original variants of TimeMoE~\cite{shi2024timemoe}, MOIRAI~\cite{woo2024moirai}, and Chronos~\cite{Chronos}. 
% 
Second, Table~\ref{domain_specific} evaluates the long-term forecasting setting on ETTh1, ETTh2, ETTm1, ETTm2, and Weather, comparing QUALS-pretrained variants with recent and classical domain-specific models, including TQNet~\cite{lin2025temporal}, OLinear~\cite{yue2026olinear}, TimeMixer~\cite{wangtimemixer}, iTransformer~\cite{liuitransformer}, TimesNet~\cite{DBLP:conf/iclr/WuHLZ0L23}, PatchTST~\cite{nietime}, TiDE~\cite{daslong}, and DLinear~\cite{zeng2023transformers}.

\noindent \respblock{Issue Q3.2 (W2, Q2):} \textit{The paper reads like a sequence of design decisions. There are no discussions of the design space and no rational given for individual design decisions. The ablation study looks back at some aspect of the design space, but there is no clear description of the design space. \& What is the rationale behind the design decisions in Section 4?}

\noindent \textbf{Response A3.2:} 
We agree and revised Section~\ref{sec:method} to organize the method around explicit design constraints rather than presenting it as a sequence of implementation choices.
% 
Stages 1–2 implement the construction policy $\pi_c$: Stage 1 creates countable multi-scale temporal units, while Stage 2 converts them into a series-level pattern space with more uniform occupancy.
% 
Stage 3 implements the sampling policy $\pi_s$, because balanced pattern counts do not guarantee balanced optimization progress across bins with different learnability.

We also connect each design choice to an evaluated alternative: handcrafted pattern representations and online weighting are compared in Table~\ref{tab:vldb_all_benchmarks_sampling_tsfm_last}, while component-removal ablations are reported in Table~\ref{tab:ablation_transposed_quals_321_best}. Responses G3.1–G3.4 summarize this design space and explain why the stages address distinct, non-interchangeable constraints.

\noindent \respblock{Issue Q3.3 (W3, Detailed Evaluation):}  \textit{Learnability is never formally defined. GRPO is mentioned but not explained in depth.}

\noindent \textbf{Response A3.3:} 
We revised Section~\ref{sec:preliminaries} to formally define the learnability of a pattern bin as the effective training budget required to reach a convergence level, and we operationalize this definition using the observed convergence speed $r_{i,t}$ under uniform probing.
% 
We also revised Section~\ref{sec:method} to explain the offline profiling procedure, the learnability-profile matrix $\mathcal{R}$, the GRPO~\cite{fu2025reward} synchronization reward, and the reason for decoupling policy optimization from forecasting-model training. 
The formal definition and optimization procedure are summarized in Response G3.3, while the offline-versus-online design choice is discussed in Response G3.4.


==> tables/alg_2.tex <==

\begin{algorithm}[t]
\small
\renewcommand{\baselinestretch}{0.85}\selectfont
\caption{Learnability Synchronization via GRPO}
\label{alg:grpo_sync}
\begin{algorithmic}[1]
\Require Bin Embeddings $\{v_i\}_{i=1}^M$, Training Budget $T_{max}$, Subset Size $B$.
\Ensure Learnability-Balanced Weights $\mathbf{w}^*$.

\State \textbf{Phase 1: Offline Learnability Profiling (Inner Loop)}
\State Initialize forecaster with Uniform Weights $\mathbf{w}_{uni}$.
\State Train model and record validation curves across stages $t$.
\State Compute stage-aware convergence speeds:
\State \quad $r_{i,t} \leftarrow \text{Slope}(\text{ValMetric}_{i,t})$ for all $i \in \{1,\dots,M\}$.

\State \textbf{Phase 2: GRPO Optimization (Outer Loop)}
\State Initialize policy $\pi_\theta$ and Group Pool $\mathcal{H} \leftarrow \emptyset$.
\For{iter $= 1$ to $T_{max}$} \Comment{Rapid optimization iterations}
    \State \textbf{Step A: Policy Modeling}
    \State Sample a random subset of bins $\mathcal{B}$ of size $B$.
    \State Sample a training stage index $t$.
    \State Compute logits $\mu \leftarrow f_\theta(\mathbf{V}_{\mathcal{B}})$ and sample weights:
    \State \quad $\mathbf{w} \leftarrow \text{Softmax}(\mu + \mathcal{N}(0, \sigma))$ 

    \State \textbf{Step B: Reward Design}
    \State Calc effective speeds $p_{i,t} \leftarrow w_i \cdot r_{i,t}$ and local mean $\bar{p}_t$.
    \State Compute Reward: $R_{i,t} \leftarrow -(p_{i,t} - \bar{p}_t)^2$ 

    \State \textbf{Step C: Group Update}
    \State Store group: $\mathcal{H} \leftarrow \mathcal{H} \cup \{(\mathcal{B}, \mathbf{R}_t)\}$.
    \State Sample $\mathcal{G} \sim \mathcal{H}$ and compute Advantage $A_{i,t}$.
    \State Update $\theta$ by minimizing clipped $\mathcal{L}_{\text{GRPO}}$.
\EndFor
\State \Return Final Weights $\mathbf{w}^* \leftarrow \text{Softmax}(f_\theta(\mathbf{V}))$
\end{algorithmic}
\end{algorithm}


==> tables/aries_test.tex <==

\begin{table*}[]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{0.cm}
\caption{
Performance comparison on ARIES TEST.
Models with superior performance are highlighted in {\color{MyRed2}\textbf{red}}.
}
\setlength\tabcolsep{1.pt}
\resizebox{1\linewidth}{!}{
\begin{tabular}{rr|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule[1.5pt]
\multicolumn{2}{l}{\textbf{Models}} & \multicolumn{1}{|l}{\textbf{TimeMoE}$_{l}^{\textbf{Q}}$} & \multicolumn{1}{l}{\textbf{TimeMoE}$_{l}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{TimeMoE}$_{l}$} &
 \multicolumn{1}{l}{\textbf{TimeMoE}$_{b}^{\textbf{Q}}$}
& \multicolumn{1}{l}{\textbf{TimeMoE}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{TimeMoE}$_{b}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{l}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{l}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{MOIRAI}$_{l}$} & 
\multicolumn{1}{l}{\textbf{MOIRAI}$_{b}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{MOIRAI}$_{b}$} 
&\multicolumn{1}{l}{\textbf{Chronos}$_{b}^{\textbf{Q}}$}
& \multicolumn{1}{l}{\textbf{Chronos}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{Chronos}$_{b}$} & 
\multicolumn{1}{l}{\textbf{Chronos}$_{s}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{Chronos}$_{s}^{\textbf{B}}$} & \multicolumn{1}{l}{\textbf{Chronos}$_{s}$} \\
\midrule
\multicolumn{2}{c|}{\textbf{MAE}$\downarrow$}  &{\color{MyRed2}\textbf{0.322}}&0.366& 0.401&{\color{MyRed2}\textbf{0.320}}& 0.343&0.363 &{\color{MyRed2}\textbf{0.363}}&0.454&0.671 &{\color{MyRed2}\textbf{0.368}}&0.494& 0.658&{\color{MyRed2}\textbf{0.303}}&0.326&0.337 &{\color{MyRed2}\textbf{0.333}}&0.337&0.339 \\
\midrule
\multicolumn{2}{c|}{\textbf{MSE}$\downarrow$}  &{\color{MyRed2}\textbf{0.353}}&0.412& 0.424&{\color{MyRed2}\textbf{0.347}}& 0.415&0.411 &{\color{MyRed2}\textbf{0.412}}&0.522&1.012 &{\color{MyRed2}\textbf{0.435}}&0.583& 2.193&{\color{MyRed2}\textbf{0.313}}&0.338&0.349 &{\color{MyRed2}\textbf{0.338}}&0.349&0.352 \\

\bottomrule[1.5pt]
\end{tabular}}
\label{tab:ARIES}
\vspace{-5pt}
\end{table*}


==> tables/comparison.tex <==

% % Requires: \usepackage{booktabs,graphicx,xcolor,multirow}
% \providecommand{\best}[1]{{\color{red}\textbf{#1}}}
% \providecommand{\second}[1]{{\color{blue}\textbf{#1}}}

% \begin{table*}[!t]
% \centering
% \setlength{\abovecaptionskip}{0.cm}
% \setlength{\belowcaptionskip}{0.cm}
% \setlength{\tabcolsep}{0.55pt}
% \caption{
% Cross-benchmark performance (LTSF: mean over horizons 96--720).
% Lower is better except FEV/TSFM skill scores.
% \best{Red} and \second{Blue}: best and second-best per model family (ChronosBolt-Small or TimeMoE-Base).
% }
% \resizebox{1\linewidth}{!}{%
% \begin{tabular}{l|cccccccccc|cc|cc|cc|cccc|cc}
% \toprule[1.5pt]
% \multirow{3}{*}{\textbf{Models}} &
% \multicolumn{10}{c|}{\textbf{LTSF}} &
% \multicolumn{2}{c|}{\textbf{ARIES-TEST}} &
% \multicolumn{2}{c|}{\textbf{GIFT-Eval-B}} &
% \multicolumn{2}{c|}{\textbf{GIFT-Eval-F}} &
% \multicolumn{4}{c|}{\textbf{FEV}} &
% \multicolumn{2}{c}{\textbf{TSFM-Bench}} \\
% \cmidrule(lr){2-11}
% \cmidrule(lr){12-13}
% \cmidrule(lr){14-15}
% \cmidrule(lr){16-17}
% \cmidrule(lr){18-21}
% \cmidrule(lr){22-23}
% &
% \multicolumn{2}{c}{\textbf{ETTh1}} &
% \multicolumn{2}{c}{\textbf{ETTh2}} &
% \multicolumn{2}{c}{\textbf{ETTm1}} &
% \multicolumn{2}{c}{\textbf{ETTm2}} &
% \multicolumn{2}{c|}{\textbf{Weather}} &
% \multicolumn{2}{c|}{\textbf{Synth}} &
% \multicolumn{2}{c|}{\textbf{Average}} &
% \multicolumn{2}{c|}{\textbf{Average}} &
% \multicolumn{4}{c|}{\textbf{Skill Score}} &
% \multicolumn{2}{c}{\textbf{Skill Score}} \\
% \cmidrule(lr){2-3}
% \cmidrule(lr){4-5}
% \cmidrule(lr){6-7}
% \cmidrule(lr){8-9}
% \cmidrule(lr){10-11}
% \cmidrule(lr){12-13}
% \cmidrule(lr){14-15}
% \cmidrule(lr){16-17}
% \cmidrule(lr){18-21}
% \cmidrule(lr){22-23}
% &
% \textbf{MSE$\downarrow$} & \textbf{MAE$\downarrow$} &
% \textbf{MSE$\downarrow$} & \textbf{MAE$\downarrow$} &
% \textbf{MSE$\downarrow$} & \textbf{MAE$\downarrow$} &
% \textbf{MSE$\downarrow$} & \textbf{MAE$\downarrow$} &
% \textbf{MSE$\downarrow$} & \textbf{MAE$\downarrow$} &
% \textbf{MSE$\downarrow$} & \textbf{MAE$\downarrow$} &
% \textbf{MASE$\downarrow$} & \textbf{CRPS$\downarrow$} &
% \textbf{MASE$\downarrow$} & \textbf{CRPS$\downarrow$} &
% \textbf{SQL$\uparrow$} & \textbf{MASE$\uparrow$} & \textbf{WQL$\uparrow$} & \textbf{WAPE$\uparrow$} &
% \textbf{MAE$\uparrow$} & \textbf{MSE$\uparrow$} \\
% \midrule

% \multicolumn{23}{c}{\textbf{ChronosBolt Small Variants}} \\
% \midrule

% \textit{Original}
% & 0.467 & 0.428
% & 0.370 & 0.385
% & 0.411 & 0.388
% & 0.291 & 0.330
% & 0.253 & 0.268
% & 0.352 & 0.339
% & 0.736 & 0.485
% & 0.822 & 0.577
% & 0.378 & 0.256 & 0.422 & 0.290
% & 0.174 & 0.391 \\

% \textit{BLAST}
% & 0.410 & 0.408
% & 0.358 & 0.382
% & 0.404 & 0.385
% & \best{0.282} & \best{0.316}
% & 0.249 & 0.268
% & 0.349 & 0.337
% & \second{0.684} & 0.470
% & \second{0.809} & \second{0.574}
% & 0.382 & 0.260 & 0.422 & 0.287
% & 0.175 & 0.393 \\

% \textit{QUALS}
% & \best{0.382} & \best{0.399}
% & \best{0.346} & \second{0.373}
% & \best{0.371} & \second{0.381}
% & \second{0.287} & \second{0.321}
% & \best{0.243} & \best{0.263}
% & \second{0.338} & \second{0.333}
% & \best{0.663} & \best{0.453}
% & \best{0.803} & \best{0.571}
% & \best{0.391} & \best{0.275} & \best{0.430} & \best{0.303}
% & \second{0.199} & \best{0.435} \\

% \textit{AvgDomain}
% & 0.419 & 0.417
% & 0.375 & 0.394
% & \second{0.382} & 0.389
% & 0.303 & 0.335
% & 0.251 & 0.268
% & 0.729 & 0.566
% & 0.755 & 0.524
% & 0.882 & 0.628
% & 0.345 & 0.218 & 0.391 & 0.249
% & \best{0.200} & \second{0.429} \\

% \textit{Catch22}
% & \second{0.398} & 0.407
% & \second{0.350} & 0.380
% & 0.679 & 0.486
% & 0.327 & 0.358
% & 0.275 & 0.290
% & 0.798 & 0.596
% & 0.793 & 0.545
% & 0.939 & 0.670
% & 0.332 & 0.198 & 0.372 & 0.226
% & 0.116 & 0.341 \\

% \textit{Online-GRPO}
% & 0.403 & \second{0.404}
% & \best{0.346} & \best{0.371}
% & 0.391 & \best{0.380}
% & 0.288 & \second{0.321}
% & \second{0.247} & \second{0.266}
% & \best{0.332} & \best{0.305}
% & 0.687 & \second{0.461}
% & 0.838 & 0.588
% & \second{0.383} & \second{0.265} & \second{0.428} & \second{0.297}
% & 0.184 & 0.417 \\

% \textit{AvgDataset}
% & 0.414 & 0.412
% & 0.355 & 0.381
% & 0.386 & 0.391
% & 0.329 & 0.351
% & 0.261 & 0.282
% & 0.794 & 0.596
% & 0.757 & 0.522
% & 0.886 & 0.629
% & 0.379 & 0.255 & 0.427 & 0.293
% & 0.126 & 0.283 \\

% \midrule
% \multicolumn{23}{c}{\textbf{TimeMoE Base Variants}} \\
% \midrule

% \textit{Original}
% & 0.400 & 0.424
% & 0.366 & 0.404
% & \second{0.394} & 0.415
% & 0.317 & 0.365
% & 0.274 & 0.297
% & 0.411 & 0.363
% & 0.888 & 0.706
% & 1.067 & 0.906
% & 0.032 & 0.040 & 0.070 & 0.056
% & -0.167& -0.060 \\

% \textit{BLAST}
% & 0.399 & 0.412
% & 0.356 & 0.391
% & \second{0.394} & 0.399
% & \second{0.274} & \second{0.326}
% & \best{0.244} & \best{0.278}
% & 0.415 & \second{0.343}
% & \second{0.760} & \second{0.616}
% & \second{0.896} & \second{0.766}
% & 0.059 & 0.067 & 0.097 & 0.083
% & 0.079 & 0.321 \\

% \textit{QUALS}
% & \best{0.383} & \best{0.405}
% & \best{0.338} & \best{0.384}
% & \best{0.354} & \best{0.378}
% & \best{0.251} & \best{0.316}
% & \second{0.248} & \second{0.282}
% & \best{0.347} & \best{0.320}
% & \best{0.734} & \best{0.593}
% & \best{0.881} & \best{0.759}
% & \second{0.094} & \second{0.102} & \best{0.123} & \best{0.109}
% & \second{0.122} & \second{0.371} \\

% \textit{AvgDomain}
% & 0.407 & 0.423
% & 0.356 & \second{0.388}
% & 0.428 & 0.417
% & 0.303 & 0.346
% & 0.257 & 0.292
% & 0.728 & 0.604
% & 1.056 & 0.811
% & 1.021 & 0.866
% & -0.022 & -0.013 & -0.000 & -0.015
% & 0.085 & 0.343 \\

% \textit{Catch22}
% & \second{0.393} & 0.413
% & 0.362 & 0.398
% & 0.688 & 0.535
% & 0.313 & 0.361
% & 0.271 & 0.307
% & 0.757 & 0.613
% & 1.066 & 0.819
% & 1.086 & 0.937
% & -0.021 & -0.011 & 0.004 & -0.011
% & 0.025 & 0.280 \\

% \textit{Online-GRPO}
% & 0.394 & \second{0.407}
% & \second{0.352} & 0.389
% & 0.397 & \second{0.391}
% & 0.276 & \second{0.326}
% & 0.255 & 0.290
% & \second{0.390} & 0.354
% & 0.841 & 0.686
% & 0.949 & 0.814
% & \best{0.095} & \best{0.103} & \second{0.118} & \second{0.105}
% & \best{0.123} & \best{0.374} \\

% \textit{AvgDataset}
% & 0.432 & 0.445
% & 0.361 & 0.391
% & 0.443 & 0.423
% & 0.314 & 0.353
% & 0.263 & 0.301
% & 0.731 & 0.604
% & 1.067 & 0.819
% & 1.031 & 0.873
% & 0.002 & 0.011 & 0.035 & 0.021
% & 0.058 & 0.319 \\

% \bottomrule[1.5pt]
% \end{tabular}%
% }
% \label{tab:vldb_all_benchmarks_sampling_tsfm_last}
% \vspace{1mm}
% \footnotesize{
% GIFT-Eval-B denotes the BLAST-configured Gift-Eval benchmark, where only leakage-free test data are retained.
% GIFT-Eval-F denotes the full Gift-Eval benchmark.
% Original, BLAST, and QUALS denote the official, BLAST-curated, and QUALS-curated variants, respectively.
% AvgDomain, Catch22, Online-GRPO, and AvgDataset denote alternative corpus sampling strategies.
% FEV and TSFM report skill scores, where larger values indicate better performance.
% }
% \end{table*}

% Requires: \usepackage{booktabs,graphicx,xcolor,multirow}
\providecommand{\best}[1]{{\color{MyRed2}\textbf{#1}}}
\providecommand{\second}[1]{{\color{MyBlue}\textbf{#1}}}

\begin{table*}[!t]
\centering
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{0.cm}
\setlength{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{0.9}
\caption{
Performance comparison of different corpus construction strategies. 
\best{Red} and \second{Blue} indicate the best and second-best results within each model family, respectively.
}
\resizebox{1\linewidth}{!}{%
\begin{tabular}{r c|cccccccccc|cc|cc|cc|cc|cccc}
\toprule[1.5pt]
\multirow{2}{*}{} & \multirow{2}{*}{\textbf{Variant}} &
\multicolumn{2}{c}{\textbf{ETTh1}} &
\multicolumn{2}{c}{\textbf{ETTh2}} &
\multicolumn{2}{c}{\textbf{ETTm1}} &
\multicolumn{2}{c}{\textbf{ETTm2}} &
\multicolumn{2}{c|}{\textbf{Weather}} &
\multicolumn{2}{c|}{\textbf{ARIES-TEST}} &
\multicolumn{2}{c|}{\textbf{GIFT-Eval-B}} &
\multicolumn{2}{c|}{\textbf{GIFT-Eval-F}} &
\multicolumn{2}{c|}{\textbf{TSFM-Bench}} &
\multicolumn{4}{c}{\textbf{FEV}} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
\cmidrule(lr){13-14}
\cmidrule(lr){15-16}
\cmidrule(lr){17-18}
\cmidrule(lr){19-20}
\cmidrule(lr){21-24}
&
&
\textbf{MSE$\downarrow$} & \textbf{MAE$\downarrow$} &
\textbf{MSE$\downarrow$} & \textbf{MAE$\downarrow$} &
\textbf{MSE$\downarrow$} & \textbf{MAE$\downarrow$} &
\textbf{MSE$\downarrow$} & \textbf{MAE$\downarrow$} &
\textbf{MSE$\downarrow$} & \textbf{MAE$\downarrow$} &
\textbf{MSE$\downarrow$} & \textbf{MAE$\downarrow$} &
\textbf{MASE$\downarrow$} & \textbf{CRPS$\downarrow$} &
\textbf{MASE$\downarrow$} & \textbf{CRPS$\downarrow$} &
\textbf{MAE$\uparrow$} & \textbf{MSE$\uparrow$} &
\textbf{SQL$\uparrow$} & \textbf{MASE$\uparrow$} & \textbf{WQL$\uparrow$} & \textbf{WAPE$\uparrow$} \\
\midrule

\multirow{7}{*}{\rotatebox{90}{$\textbf{ChronosBolt}_s$}}
& {Original}
& .467 & .428
& .370 & .385
& .411 & .388
& .291 & .330
& .253 & .268
& .352 & .339
& .736 & .485
& .822 & .577
& .174 & .391
& .378 & .256 & .422 & .290 \\

& {AvgDataset}
& .414 & .412
& .355 & .381
& .386 & .391
& .329 & .351
& .261 & .282
& .794 & .596
& .757 & .522
& .886 & .629
& .126 & .283
& .379 & .255 & .427 & .293 \\

& {AvgDomain}
& .419 & .417
& .375 & .394
& \second{.382} & .389
& .303 & .335
& .251 & .268
& .729 & .566
& .755 & .524
& .882 & .628
& \best{.200} & \second{.429}
& .345 & .218 & .391 & .249 \\

& {Catch22}
& \second{.398} & .407
& \second{.350} & .380
& .679 & .486
& .327 & .358
& .275 & .290
& .798 & .596
& .793 & .545
& .939 & .670
& .116 & .341
& .332 & .198 & .372 & .226 \\

& {BLAST}
& .410 & .408
& .358 & .382
& .404 & .385
& \best{.282} & \best{.316}
& .249 & .268
& .349 & .337
& \second{.684} & .470
& \second{.809} & \second{.574}
& .175 & .393
& .382 & .260 & .422 & .287 \\

& {Online-GRPO}
& .403 & \second{.404}
& \best{.346} & \best{.371}
& .391 & \best{.380}
& .288 & \second{.321}
& \second{.247} & \second{.266}
& \best{.332} & \best{.305}
& .687 & \second{.461}
& .838 & .588
& .184 & .417
& \second{.383} & \second{.265} & \second{.428} & \second{.297} \\

% \rowcolor{tabhighlight}\cellcolor{white}
\rowcolor{blue!15}\cellcolor{white!0}
& {QUALS}
& \best{.382} & \best{.399}
& \best{.346} & \second{.373}
& \best{.371} & \second{.381}
& \second{.287} & \second{.321}
& \best{.243} & \best{.263}
& \second{.338} & \second{.333}
& \best{.663} & \best{.453}
& \best{.803} & \best{.571}
& \second{.199} & \best{.435}
& \best{.391} & \best{.275} & \best{.430} & \best{.303} \\

\midrule

\multirow{7}{*}{\rotatebox{90}{$\textbf{TimeMoE}_{b}$}}

& {Original}
& .400 & .424
& .366 & .404
& \second{.394} & .415
& .317 & .365
& .274 & .297
& .411 & .363
& .888 & .706
& 1.067 & .906
& -0.167& -0.060
& .032 & .040 & .070 & .056 \\

& {AvgDataset}
& .432 & .445
& .361 & .391
& .443 & .423
& .314 & .353
& .263 & .301
& .731 & .604
& 1.067 & .819
& 1.031 & .873
& .058 & .319
& .002 & .011 & .035 & .021 \\

& {AvgDomain}
& .407 & .423
& .356 & \second{.388}
& .428 & .417
& .303 & .346
& .257 & .292
& .728 & .604
& 1.056 & .811
& 1.021 & .866
& .085 & .343
& -0.022 & -0.013 & -0.000 & -0.015 \\

& {Catch22}
& \second{.393} & .413
& .362 & .398
& .688 & .535
& .313 & .361
& .271 & .307
& .757 & .613
& 1.066 & .819
& 1.086 & .937
& .025 & .280
& -0.021 & -0.011 & .004 & -0.011 \\

& {BLAST}
& .399 & .412
& .356 & .391
& \second{.394} & .399
& \second{.274} & \second{.326}
& \best{.244} & \best{.278}
& .415 & \second{.343}
& \second{.760} & \second{.616}
& \second{.896} & \second{.766}
& .079 & .321
& .059 & .067 & .097 & .083 \\

& {Online-GRPO}
& .394 & \second{.407}
& \second{.352} & .389
& .397 & \second{.391}
& .276 & \second{.326}
& .255 & .290
& \second{.390} & .354
& .841 & .686
& .949 & .814
& \best{.123} & \best{.374}
& \best{.095} & \best{.103} & \second{.118} & \second{.105} \\

% \rowcolor{tabhighlight}\cellcolor{white}
% \rowcolor{tabhighlight}\cellcolor{white}
% \cellcolor{white}
\rowcolor{blue!15}\cellcolor{white!0}
& 
{QUALS}
& \best{.383} & \best{.405}
& \best{.338} & \best{.384}
& \best{.354} & \best{.378}
& \best{.251} & \best{.316}
& \second{.248} & \second{.282}
& \best{.347} & \best{.320}
& \best{.734} & \best{.593}
& \best{.881} & \best{.759}
& \second{.122} & \second{.371}
& \second{.094} & \second{.102} & \best{.123} & \best{.109} \\

\bottomrule[1.5pt]
\end{tabular}%
}
\label{tab:vldb_all_benchmarks_sampling_tsfm_last}
\end{table*}


==> tables/domain_specific.tex <==
\begin{table*}[!t]
\setlength{\abovecaptionskip}{0.cm}
\caption{
Comparison of zero-shot models pretrained on QUALS and domain-specific models. 
{\color{MyRed2}\textbf{Red}} and {\color{MyBlue}Blue} indicate the best and second-best results, respectively.
% Comparison of zero-shot QUALS models and domain-specific models. {\color{MyRed2}\textbf{Red}}: best, {\color{MyBlue}Blue}: 2nd best.
}
\setlength\tabcolsep{1.5pt}
\renewcommand{\arraystretch}{0.9}
\resizebox{1\linewidth}{!}{%
\begin{tabular}{rr|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}
\toprule[1.5pt]
\multicolumn{2}{l}{} & \multicolumn{12}{c}{\textbf{Pre-training on QUALS}} & \multicolumn{16}{c}{\textbf{Domain-specific Models}}\\
\cmidrule(r){3-14} \cmidrule(r){15-30}
\multicolumn{2}{r}{\textbf{Models}} & \multicolumn{2}{|c}{\textbf{TimeMoE}$_{b}^{\textbf{Q}}$} & \multicolumn{2}{c|}{\textbf{TimeMoE}$_{l}^{\textbf{Q}}$} & \multicolumn{2}{c|}{\textbf{MOIRAI}$_{b}^{\textbf{Q}}$} & \multicolumn{2}{c|}{\textbf{MOIRAI}$_{l}^{\textbf{Q}}$} & \multicolumn{2}{c|}{\textbf{Chronos}$_{b}^{\textbf{Q}}$} & \multicolumn{2}{c|}{\textbf{Chronos}$_{s}^{\textbf{Q}}$} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{TQNet}\\2025~\cite{lin2025temporal}\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{OLinear}\\2025~\cite{yue2026olinear}\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{TimeMixer}\\2024~\cite{wangtimemixer}\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{iTransformer}\\2024~\cite{liuitransformer}\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{TimesNet}\\2023~\cite{DBLP:conf/iclr/WuHLZ0L23}\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{PatchTST}\\2023~\cite{nietime}\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{TiDE}\\2023~\cite{daslong}\end{tabular}}& \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{DLinear}\\2023~\cite{zeng2023transformers}\end{tabular}} \\
\cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10} \cmidrule(r){11-12} \cmidrule(r){13-14} \cmidrule(r){15-16} \cmidrule(r){17-18} \cmidrule(r){19-20} \cmidrule(r){21-22} \cmidrule(r){23-24} \cmidrule(r){25-26} \cmidrule(r){27-28} \cmidrule(r){29-30}
\multicolumn{2}{r|}{\textbf{Metrics}} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} \\
\midrule
\multicolumn{2}{r|}{\rotatebox{0}{ETTh1}}
&\color{MyBlue}\textbf{.383}&.405&.389&.408&.407&.408&.401&.404&.391&\color{MyBlue}\textbf{.401}&\color{MyRed2}\textbf{.382}&\color{MyRed2}\textbf{.399}&.437&.433&.444&.446&.448&.442&.454&.447&.454&.450&.468&.454&.540&.507&.455&.451\\
\multicolumn{2}{r|}{\rotatebox{0}{ETTh2}}
&\color{MyRed2}\textbf{.338}&.384&.345&.387&.344&\color{MyRed2}\textbf{.369}&\color{MyBlue}\textbf{.341}&\color{MyBlue}\textbf{.370}&.349&.374&.346&.373&.390&.417&.393&.420&.364&.395&.383&.406&.414&.496&.386&.406&.611&.549&.558&.515\\
\multicolumn{2}{r|}{\rotatebox{0}{ETTm1}}
&.354&.378&\color{MyRed2}\textbf{.346}&.375&.377&.378&.386&.377&.390&.379&.371&.381&.355&\color{MyRed2}\textbf{.371}&\color{MyBlue}\textbf{.350}&\color{MyBlue}\textbf{.374}&.381&.395&.407&.409&.400&.405&.387&.400&.419&.419&.403&.406\\
\multicolumn{2}{r|}{\rotatebox{0}{ETTm2}}
&\color{MyBlue}\textbf{.251}&.316&\color{MyRed2}\textbf{.243}&\color{MyBlue}\textbf{.310}&.274&.317&.259&\color{MyRed2}\textbf{.303}&.275&.313&.287&.321&.259&.312&.263&.314&.275&.323&.288&.332&.291&.332&.280&.326&.358&.403&.350&.400\\
\multicolumn{2}{r|}{\rotatebox{0}{Weather}}
&.248&.282&.248&.280&.258&.272&.247&.265&.240&.259&.243&.263&\color{MyRed2}\textbf{.221}&\color{MyRed2}\textbf{.249}&\color{MyBlue}\textbf{.226}&\color{MyBlue}\textbf{.250}&.240&.271&.257&.278&.258&.286&.258&.280&.270&.320&.265&.316\\
\midrule
\rowc\rowcolor{blue!15}
\multicolumn{2}{c|}{\scalebox{1.1}{\textbf{Average}}}
&{\color{MyBlue}\textbf{.315}}&.353&{\color{MyRed2}\textbf{.314}}&.352&.332&.349&.327&{\color{MyRed2}\textbf{.344}}&.329&{\color{MyBlue}\textbf{.345}}&.326&.347&.332&.356&.335&.361&.342&.365&.358&.374&.363&.394&.356&.373&.440&.440&.406&.418\\
\bottomrule[1.5pt]
\end{tabular}}
\label{domain_specific}
\end{table*}


==> tables/fev_bench.tex <==

\begin{table*}[]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{0.cm}
\vspace{-5pt}
\caption{
Performance of Skill Score on Fev benchmark.
Models with superior performance are highlighted in {\color{MyRed2}\textbf{red}}.
}
\setlength\tabcolsep{1.pt}
\resizebox{1\linewidth}{!}{
\begin{tabular}{rr|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule[1.5pt]
\multicolumn{2}{l}{\textbf{Models}} & \multicolumn{1}{|l}{\textbf{TimeMoE}$_{l}^{\textbf{Q}}$} & \multicolumn{1}{l}{\textbf{TimeMoE}$_{l}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{TimeMoE}$_{l}$} &
 \multicolumn{1}{l}{\textbf{TimeMoE}$_{b}^{\textbf{Q}}$}
& \multicolumn{1}{l}{\textbf{TimeMoE}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{TimeMoE}$_{b}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{l}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{l}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{MOIRAI}$_{l}$} & 
\multicolumn{1}{l}{\textbf{MOIRAI}$_{b}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{MOIRAI}$_{b}$} 
&\multicolumn{1}{l}{\textbf{Chronos}$_{b}^{\textbf{Q}}$}
& \multicolumn{1}{l}{\textbf{Chronos}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{Chronos}$_{b}$} & 
\multicolumn{1}{l}{\textbf{Chronos}$_{s}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{Chronos}$_{s}^{\textbf{B}}$} & \multicolumn{1}{l}{\textbf{Chronos}$_{s}$} \\
\midrule
\multicolumn{2}{c|}{\textbf{SQL}$\uparrow$}  &{\color{MyRed2}\textbf{0.102}}&0.086&0.035 &{\color{MyRed2}\textbf{0.094}}&0.059& 0.032&{\color{MyRed2}\textbf{0.360}}&0.303&0.351&{\color{MyRed2}\textbf{0.350}}&0.292&0.321 &{\color{MyRed2}\textbf{0.393}}&0.386& 0.389&{\color{MyRed2}\textbf{0.391}}&0.382&0.378 \\
\midrule
\multicolumn{2}{c|}{\textbf{MASE}$\uparrow$}  &{\color{MyRed2}\textbf{0.110}}&0.095& 0.044&{\color{MyRed2}\textbf{0.102}}&0.067&0.040 &{\color{MyRed2}\textbf{0.226}}&0.151& 0.216&{\color{MyRed2}\textbf{0.214}}&0.140& 0.181&{\color{MyRed2}\textbf{0.275}}&0.266& 0.265&{\color{MyRed2}\textbf{0.275}}&0.260&0.256\\
\midrule
\multicolumn{2}{c|}{\textbf{WQL}$\uparrow$}  &{\color{MyRed2}\textbf{0.138}}&0.113&0.088 &{\color{MyRed2}\textbf{0.123}}&0.097&0.070 &0.398&0.352& {\color{MyRed2}\textbf{0.405}}&{\color{MyRed2}\textbf{0.388}}&0.338& 0.374&{\color{MyRed2}\textbf{0.437}}&0.428& 0.432&{\color{MyRed2}\textbf{0.430}}&0.422&0.422 \\
\midrule
\multicolumn{2}{c|}{\textbf{WAPE}$\uparrow$} 
 &{\color{MyRed2}\textbf{0.125}}&0.100&0.075 &{\color{MyRed2}\textbf{0.109}}&0.083&0.056 &0.247&0.192& {\color{MyRed2}\textbf{0.259}}&{\color{MyRed2}\textbf{0.236}}&0.175& 0.228&{\color{MyRed2}\textbf{0.307}}&0.296& 0.298&{\color{MyRed2}\textbf{0.303}}&0.287&0.290\\

\bottomrule[1.5pt]
\end{tabular}}
\label{tab:fev}
\end{table*}


==> tables/gift_eval.tex <==

\begin{table*}[]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{0.cm}
\caption{
Performance on full Gift-Eval benchmark.
Models with superior performance are highlighted in {\color{MyRed2}\textbf{red}}.
}
\setlength\tabcolsep{1.pt}
\resizebox{1\linewidth}{!}{
\begin{tabular}{rr|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule[1.5pt]
\multicolumn{2}{l}{\textbf{Models}} & \multicolumn{1}{|l}{\textbf{TimeMoE}$_{l}^{\textbf{Q}}$} & \multicolumn{1}{l}{\textbf{TimeMoE}$_{l}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{TimeMoE}$_{l}$} &
 \multicolumn{1}{l}{\textbf{TimeMoE}$_{b}^{\textbf{Q}}$}
& \multicolumn{1}{l}{\textbf{TimeMoE}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{TimeMoE}$_{b}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{l}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{l}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{MOIRAI}$_{l}$} & 
\multicolumn{1}{l}{\textbf{MOIRAI}$_{b}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{MOIRAI}$_{b}$} 
&\multicolumn{1}{l}{\textbf{Chronos}$_{b}^{\textbf{Q}}$}
& \multicolumn{1}{l}{\textbf{Chronos}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{Chronos}$_{b}$} & 
\multicolumn{1}{l}{\textbf{Chronos}$_{s}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{Chronos}$_{s}^{\textbf{B}}$} & \multicolumn{1}{l}{\textbf{Chronos}$_{s}$} \\
\midrule
\multicolumn{2}{c|}{\textbf{MASE}$\downarrow$} &{\color{MyRed2}\textbf{0.846}} & 0.852& 1.110& {\color{MyRed2}\textbf{0.881}}& 0.896& 1.067& {\color{MyRed2}\textbf{0.858}}& 0.880&  0.875&{\color{MyRed2}\textbf{0.888}}& 0.908& 	
0.901& {\color{MyRed2}\textbf{0.798}}& 0.804& 0.808& {\color{MyRed2}\textbf{0.803}}&0.809&0.822  \\
\midrule
\multicolumn{2}{c|}{\textbf{CRPS}$\downarrow$} & {\color{MyRed2}\textbf{0.723}}& 0.728& 0.882& {\color{MyRed2}\textbf{0.759}}& 0.766& 0.906& {\color{MyRed2}\textbf{0.580}}& 0.598& 0.599& {\color{MyRed2}\textbf{0.608}}& 0.623& 0.610& {\color{MyRed2}\textbf{0.568}}& 0.574& 0.574 & {\color{MyRed2}\textbf{0.571}}& 0.574& 0.577 \\

\bottomrule[1.5pt]
\end{tabular}}
\label{tab:gift_eval_all}
\end{table*}


==> tables/gift_eval_blast.tex <==

\begin{table*}[]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{0.cm}
\caption{
Performance comparison on the BLAST-configured GIFT-Eval benchmark.
Due to the experimental setup, we retain only the test data that do not exhibit data leakage.
Models with superior performance are highlighted in {\color{MyRed2}\textbf{red}}.
}
\setlength\tabcolsep{1.pt}
\resizebox{1\linewidth}{!}{
\begin{tabular}{rr|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule[1.5pt]
\multicolumn{2}{l}{\textbf{Models}} & \multicolumn{1}{|l}{\textbf{TimeMoE}$_{l}^{\textbf{Q}}$} & \multicolumn{1}{l}{\textbf{TimeMoE}$_{l}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{TimeMoE}$_{l}$} &
 \multicolumn{1}{l}{\textbf{TimeMoE}$_{b}^{\textbf{Q}}$}
& \multicolumn{1}{l}{\textbf{TimeMoE}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{TimeMoE}$_{b}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{l}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{l}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{MOIRAI}$_{l}$} & 
\multicolumn{1}{l}{\textbf{MOIRAI}$_{b}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{MOIRAI}$_{b}$} 
&\multicolumn{1}{l}{\textbf{Chronos}$_{b}^{\textbf{Q}}$}
& \multicolumn{1}{l}{\textbf{Chronos}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{Chronos}$_{b}$} & 
\multicolumn{1}{l}{\textbf{Chronos}$_{s}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{Chronos}$_{s}^{\textbf{B}}$} & \multicolumn{1}{l}{\textbf{Chronos}$_{s}$} \\
\midrule
\multicolumn{2}{c|}{\textbf{MASE}$\downarrow$} & {\color{MyRed2}\textbf{0.677}}&\scalebox{1.1}0.742 & 0.872 & \scalebox{1.1}
{\color{MyRed2}\textbf{0.734}}&
0.760 & 0.888 & \scalebox{1.1}
{\color{MyRed2}\textbf{0.729}}&
0.740 & 0.816 & \scalebox{1.1}
{\color{MyRed2}\textbf{0.745}}&
0.759 & 0.812 & \scalebox{1.1}
{\color{MyRed2}\textbf{0.659}} &
0.682 & 0.724 & \scalebox{1.1}
{\color{MyRed2}\textbf{0.663}}&
0.684& 0.736 \\
\midrule
\multicolumn{2}{c|}{\textbf{CRPS}$\downarrow$} &
{\color{MyRed2}\textbf{0.557}} & 0.593 & 0.702&
{\color{MyRed2}\textbf{0.593}} & 0.616 & 0.706&
{\color{MyRed2}\textbf{0.576}} & 0.580 & 0.642&
{\color{MyRed2}\textbf{0.585}} & 0.614 & 0.641&
{\color{MyRed2}\textbf{0.450}} & 0.468  & 0.489&
{\color{MyRed2}\textbf{0.453}} & 0.470 & 0.485\\

\bottomrule[1.5pt]
\end{tabular}}
\label{tab:gift_eval}
\vspace{-5pt}
\end{table*}


==> tables/response_token_budget.tex <==
\begin{table}[!t]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{0.cm}
\renewcommand\arraystretch{1.0}
\centering
\caption{
Pre-training token budgets (B) for strategies in Table~\ref{tab:vldb_all_benchmarks_sampling_tsfm_last}.
% 
\textbf{Bold}: minimum per model family;
% 
``---'': the pretraining budgets is not disclosed.
% The official ChronosBolt has not reported on it.
}
\label{tab:response_token_budget}
\small
\setlength{\tabcolsep}{5.5pt}
\begin{tabular}{l|cc}
\toprule[1.2pt]
\textbf{Strategy} & \textbf{ChronosBolt-S} & \textbf{TimeMoE-B} \\
\midrule
\textit{Original} & --- & 419.43 \\
\textit{BLAST} & 104.85 & 78.64 \\
\textit{AvgDataset} & 104.85 & 78.64 \\
\textit{AvgDomain} & 104.85 & 78.64 \\
\textit{Catch22} & 104.85 & 78.64 \\
\textit{Online-GRPO} & \textbf{61.86} & \textbf{26.20} \\
\textit{QUALS} & \textbf{61.86} & \textbf{26.20} \\
\bottomrule[1.2pt]
\end{tabular}
\end{table}


==> tables/tsfm_bench.tex <==

\begin{table*}[!t]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{0.cm}
\vspace{-5pt}
\caption{
Performance of Skill Score on TSFM benchmark.
Models with superior performance are highlighted in {\color{MyRed2}\textbf{red}}.
}
\setlength\tabcolsep{1.pt}
\resizebox{1\linewidth}{!}{
\begin{tabular}{rr|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule[1.5pt]
\multicolumn{2}{l}{\textbf{Models}} & \multicolumn{1}{|l}{\textbf{TimeMoE}$_{l}^{\textbf{Q}}$} & \multicolumn{1}{l}{\textbf{TimeMoE}$_{l}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{TimeMoE}$_{l}$} &
 \multicolumn{1}{l}{\textbf{TimeMoE}$_{b}^{\textbf{Q}}$}
& \multicolumn{1}{l}{\textbf{TimeMoE}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{TimeMoE}$_{b}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{l}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{l}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{MOIRAI}$_{l}$} & 
\multicolumn{1}{l}{\textbf{MOIRAI}$_{b}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{MOIRAI}$_{b}$} 
&\multicolumn{1}{l}{\textbf{Chronos}$_{b}^{\textbf{Q}}$}
& \multicolumn{1}{l}{\textbf{Chronos}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{Chronos}$_{b}$} & 
\multicolumn{1}{l}{\textbf{Chronos}$_{s}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{Chronos}$_{s}^{\textbf{B}}$} & \multicolumn{1}{l}{\textbf{Chronos}$_{s}$} \\
\midrule
\multicolumn{2}{c|}{\textbf{MAE}$\uparrow$}  &{\color{MyRed2}\textbf{0.139}}&0.111&-0.138 &{\color{MyRed2}\textbf{0.122}}&0.079&-0.167 &{\color{MyRed2}\textbf{0.154}}&0.153&0.103 &{\color{MyRed2}\textbf{0.162}}&0.151&0.117 &{\color{MyRed2}\textbf{0.215}}&0.050&0.188 &{\color{MyRed2}\textbf{0.199}}&0.175&0.174 \\
\midrule
\multicolumn{2}{c|}{\textbf{MSE}$\uparrow$}  &{\color{MyRed2}\textbf{0.387}}&0.362&-0.017 &{\color{MyRed2}\textbf{0.371}}&0.321&-0.060 &{\color{MyRed2}\textbf{0.368}}&0.360&0.202 &{\color{MyRed2}\textbf{0.365}}&0.346&0.258 &{\color{MyRed2}\textbf{0.442}}&0.268&0.387 &{\color{MyRed2}\textbf{0.435}}&0.393&0.391 \\
\bottomrule[1.5pt]
\end{tabular}}
\label{tab:tsfm}
\end{table*}


==> tables/tsfm_bench_main.tex <==

\begin{table*}[]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{0.cm}
\vspace{-5pt}
\caption{
Performance of Skill Score on TSFM benchmark.
Models with superior performance are highlighted in {\color{MyRed2}\textbf{red}}.
}
\setlength\tabcolsep{1.pt}
\resizebox{1\linewidth}{!}{
\begin{tabular}{rr|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule[1.5pt]
\multicolumn{2}{l}{\textbf{Models}} & \multicolumn{1}{|l}{\textbf{TimeMoE}$_{l}^{\textbf{Q}}$} & \multicolumn{1}{l}{\textbf{TimeMoE}$_{l}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{TimeMoE}$_{l}$} &
 \multicolumn{1}{l}{\textbf{TimeMoE}$_{b}^{\textbf{Q}}$}
& \multicolumn{1}{l}{\textbf{TimeMoE}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{TimeMoE}$_{b}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{l}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{l}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{MOIRAI}$_{l}$} & 
\multicolumn{1}{l}{\textbf{MOIRAI}$_{b}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{MOIRAI}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{MOIRAI}$_{b}$} 
&\multicolumn{1}{l}{\textbf{Chronos}$_{b}^{\textbf{Q}}$}
& \multicolumn{1}{l}{\textbf{Chronos}$_{b}^\textbf{B}$} & \multicolumn{1}{l|}{\textbf{Chronos}$_{b}$} & 
\multicolumn{1}{l}{\textbf{Chronos}$_{s}^{\textbf{Q}}$} &
\multicolumn{1}{l}{\textbf{Chronos}$_{s}^{\textbf{B}}$} & \multicolumn{1}{l}{\textbf{Chronos}$_{s}$} \\
\midrule
\multicolumn{2}{c|}{\textbf{MAE}$\uparrow$}  &{\color{MyRed2}\textbf{0.139}}&0.111&-0.138 &{\color{MyRed2}\textbf{0.122}}&0.079&-0.167 &{\color{MyRed2}\textbf{0.154}}&0.153&0.103 &{\color{MyRed2}\textbf{0.162}}&0.151&0.117 &{\color{MyRed2}\textbf{0.215}}&0.050&0.188 &{\color{MyRed2}\textbf{0.199}}&0.175&0.174 \\
\midrule
\multicolumn{2}{c|}{\textbf{MSE}$\uparrow$}  &{\color{MyRed2}\textbf{0.387}}&0.362&-0.017 &{\color{MyRed2}\textbf{0.371}}&0.321&-0.060 &{\color{MyRed2}\textbf{0.368}}&0.360&0.202 &{\color{MyRed2}\textbf{0.365}}&0.346&0.258 &{\color{MyRed2}\textbf{0.442}}&0.268&0.387 &{\color{MyRed2}\textbf{0.435}}&0.393&0.391 \\
\bottomrule[1.5pt]
\end{tabular}}
\label{tab:tsfm_main}
\end{table*}

